An Iterated Az\'{e}ma-Yor Type Embedding for Finitely Many Marginals

We solve the $n$-marginal Skorokhod embedding problem for a continuous local martingale and a sequence of probability measures $\mu_1,...,\mu_n$ which are in convex order and satisfy an additional technical assumption. Our construction is explicit and is a multiple marginal generalisation of the Azema and Yor (1979) solution. In particular, we recover the stopping boundaries obtained by Brown et al. (2001) and Madan and Yor (2002). Our technical assumption is necessary for the explicit embedding, as demonstrated with a counterexample. We discuss extensions to the general case giving details when $n=3$. In our analysis we compute the law of the maximum at each of the n stopping times. This is used in Henry-Labordere et al. (2013) to show that the construction maximises the distribution of the maximum among all solutions to the $n$-marginal Skorokhod embedding problem. The result has direct implications for robust pricing and hedging of Lookback options.

==> LP_intuition.tex <==


 
\subsection{Intuition from Linear Programming, $n=3$} 
 
\subsubsection{Static Position in Calls}

LP suggests the following guess for the static position.

\begin{alignat}{3}
 &\lambda_1 C_1(80) &&-\lambda_2 C_1(100) \nonumber  \\
+&\lambda_2 C_2(100)&&-\lambda_1 C_2(70)  \nonumber  \\
+&\lambda_2 C_3(70) &&
\label{eq:lb_static}
\end{alignat}
where
\begin{align}
&\lambda_1>\lambda_2>0, \\
&\lambda_2 - \frac{1}{y-70}>0 \\
&\frac{\lambda_2 - \frac{1}{y-70}}{\lambda_1} \approx \mathrm{const.} \quad \forall y.
\end{align}

This static portfolio is robust to the choice of $y$. 
Hence, there is hope for generalizing \eqref{eq:lb_static} to something like
\begin{alignat}{3}
 &\lambda_1(\zeta) C_1(\xi_1(y)) &&-\lambda_2(\zeta) C_1(\beta_2) \nonumber  \\
+&\lambda_2(\zeta) C_2(\beta_2)  &&-\lambda_1(\zeta) C_2(\zeta)  \nonumber \\
+&\lambda_2(\zeta) C_3(\zeta) &&
\label{eq:lb_static_generalization}
\end{alignat}
and determine $\tilde{\xi}_3(y)$ by minimizing the cost of \eqref{eq:lb_static_generalization} over $\zeta \in (\alpha_2, \beta_2)$ (jump interval of $\xi_2$).

 

  

==> Nizar.tex <==

\section{Email Nizar}

\subsection{Jan's Question }

my student has been reading and studying your paper on $n$ marginales and there are some sticky points where we do not entirely see the arguments.

We will think more to catch up with what is not said but among things to highlight:

-- (proof of Thm 4.1) I do not agree with your embedding proof. I do not see really how you want to iterate BHR and certainly not how this follows from your objects. As an example, consider $n$ laws with IMRV property. Then (as you show in one corollary) you will have all $\zeta$ equal to inverse of $b_n$ and hence also all $\psi$ bars -- effectively your embedding will embed the first marginal and then the last one. I do not see how you fabricate the intermediate ones. It seems that you keep forgetting part of the domain through the restriction that things are ordered -- you can do this for optimality since the forgotten bits are irrelevant but not if you want to embed the intermediate laws. Or are we missing something?

-- I do not quite see how you enforce ordering among zetas. In particular in the proof of Lemma 4.6 when you write (4.30) you may get $\zeta_i<\zeta_{i-1}$ no?


\subsection{Nizar's Response }
Jan: the iteration of BHR is done by using $\psi_i=b_i^{-1}$ (and not $\bar{\psi_i}$) at each step. So I do not see any issue of forgetting part of the domain. Am I missing something?

As for your second point. Suppose $n=2$. Notice that $\zeta_1^*=b_1^{-1}\wedge\zeta_2$ depends on $\zeta_2$ and is by definition less than $\zeta_2$. At Step 2 of the induction, we obtain $\zeta_2^*$, and then substitute backward to get all $\zeta_1^*=b_1^{-1}\wedge\zeta^*_2$.
For the general case, all $\zeta_i^*$'s are determined at each step as a function of $\zeta_{i+1}$ which is less that $\zeta_{i+1}$. So again at the end of the induction, $\zeta_n^*$ is determined, and we deduce all $\zeta_i^*$ by substituting backward. Do you agree?
 

\subsection{Draft Email}

\begin{itemize}
	\item First point (problems with embedding argument; stopping boundaries)
		\begin{itemize}
			\item One key step in proving BHR is to run excursions from $b_1^{-1}=\psi_1$ to $\psi_2$. At time $1$ there is a one-to-one relation between $M^*_1$ and $\bar{M}^*_1$. This is no longer true in general for time $i \geq 2$, i.e. for fixed $\bar{M}^*_i$ there are in general $i$ possible positions for $M^*_i$ (ignoring even more positions coming from the stopping times $\tau'_i, i=2,\dots,n-1$). 
			
			It is not clear to us why the BHR-iteration works. 
			\item What we meant by forgetting part of the domain is the following. To illustrate the point suppose that the IMRV-property holds. In Corollary 4.1 you show $\zeta^*_n=b_n^{-1}$. In section 4.3 you describe how to define $\psi^*$. In this example several choices of $\psi_i^*$ are possible, e.g. $\psi_i^*=b_i^{-1}$ or $\psi_i^*=b_n^{-1}$.   
		\end{itemize}
	\item Second point
		\begin{itemize}
			\item Going from $n-1 \to n$ and using backward substitution, what if $\psi^n_i \neq \psi^{n-1}_i$ for some $i=1,\dots,n-1$, i.e. do we still have $M^*_i \sim \mu_i$?
		\end{itemize}
\end{itemize}

==> application_to_lookback.tex <==

\section{Application to the Lookback Option}

\subsection{Robust Superhedging}

\begin{Theorem}[Robust Superhedging -- Lookback Option]
\label{thm:Robust Hedging -- Lookback Option}
Fix $n \in \N$.
Let $G \in C^1\left([0,\infty);\R \right)$ be increasing and 
let $(M_t)_{t \leq n}$ be a stochastic process such that $0<M_0<y$.

Then
\begin{alignat}{3}
G(\bar{M}_n) \leq  G(\bar{M}_0)+ \int_{\bar{M}_0}^{\infty} & \left\{ \vphantom{ \int_{\bar{M}_0}^{\infty} \left \{ \sum_{i=1}^{n}\left( \frac{C_{\jmath_i}(\xi_{\jmath_i})}{y-\xi_{\jmath_i}} +\indicator{\bar{M}_{\jmath_{i-1}}<y,\bar{M}_{\jmath_i}\geq y, \jmath_i \neq 0} \frac{y-M_{\jmath_i}}{y-\xi_{\jmath_i}} \right) \right. } \right. && \sum_{i=1}^{n}\left( \frac{C_{\jmath_i(y)}(\xi_{\jmath_i(y)})}{y-\xi_{\jmath_i(y)}} +\indicator{\bar{M}_{\jmath_{i-1}(y)}<y,\bar{M}_{\jmath_i(y)}\geq y, \jmath_i(y) \neq 0} \frac{y-M_{\jmath_i(y)}}{y-\xi_{\jmath_i(y)}} \right)  \nonumber \\ 
															 - &  && \sum_{i=1}^{n-1}\left( \frac{C_{\jmath_i(y)}(\xi_{\jmath_{i+1}(y)})}{y-\xi_{\jmath_{i+1}(y)}} + \indicator{\bar{M}_{\jmath_i(y)} \geq y, M_{\jmath_i(y)} \geq \xi_{\jmath_{i+1}(y)}, \jmath_i(y) \neq 0} \frac{M_{\jmath_{i+1}(y)}-M_{\jmath_i(y)}}{y-\xi_{\jmath_{i+1}(y)}} \right) \left. \vphantom{ \int_{\bar{M}_0}^{\infty} \left \{ \sum_{i=1}^{n}\left( \frac{C_{\jmath_i}(\xi_{\jmath_{i+1}})}{y-\xi_{\jmath_{i+1}}} + \indicator{\bar{M}_{\jmath_i} \geq y, M_{\jmath_i} \geq \xi_{\jmath_{i+1}}, \jmath_i \neq 0} \frac{M_{\jmath_{i+1}}-M_{\jmath_i}}{y-\xi_{\jmath_{i+1}}} \right) \right. } \right\} G'(y) \dd y.
\label{eq:thm_Trajectorial_Inequality_Lookback} 
\end{alignat}
\end{Theorem}
\begin{proof}
This is a direct consequence of Theorem \ref{lem:Trajectorial_Inequality_Unordered_Case}.
\end{proof}

\subsection{Upper Price Bound}

\begin{Theorem}[Robust Upper Price Bound -- Lookback Option]
Fix $n\in \N$.
Let $(M_t)_{t\leq n}$ be a right-continuous martingale such that $0<M_0<y $ and $M_i \sim \mu_i, i=1,\dots,n$. 
Let $G \in C^1\left([0,\infty);\R \right)$ be increasing. 

Then
\begin{align}
\E{ G(\bar{M}_n) } \leq  G(\bar{M}_0)+   \int_{\bar{M}_0}^{\infty}  \sum_{i=1}^{n}\left\{  \frac{c_{\jmath_i(y)}(\xi_{\jmath_i(y)})}{y-\xi_{\jmath_i(y)}} - \frac{c_{\jmath_i(y)}(\xi_{\jmath_{i+1}(y)})}{y-\xi_{\jmath_{i+1}(y)}} \indicator{i<n} \right\} G'(y)  \dd y.
\label{eq:thm_pricing_Lookback} 					
\end{align}
\end{Theorem}

\begin{proof}
This is a direct consequence of Theorem \ref{thm:Robust Hedging -- Lookback Option}.
\end{proof}

==> conclusion.tex <==

\section{Conclusion}
\label{sec:conclusion}

In this article we proposed in a special case of $n$ measures how an iterated embedding in the spirit of \cite{AzemaYor1} and \cite{Brown98themaximum} looks like.
Optimality properties of our embedding are investigated in our parallel work \cite{Touzi_maxmax}.

We hope that our article contains some useful ideas and might motivate or inspire research in one of the following directions. 
It is a natural question to ask in which sense an iteration of other classical embeddings with optimality properties exists and which optimality properties the iterated embedding inherits. Interesting embeddings to study are certainly the Perkins and Root embeddings. 

Our work could be the starting point of a similar construction as in \cite{Rogers:93} in order to characterize all terminal joint laws of Brownian Motion and its maximum, subject to $n$ marginal law constraints.

==> extensions.tex <==



\section{Discussion of Assumption \ref{ass:unicity_minimizers} and Extensions}
\label{sec:Extensions}

In this section we present a simple example of probability measures $\mu_1,\mu_2,\mu_3$ which violate Assumption \ref{ass:unicity_minimizers} and where the stopping boundaries $\xi_1,\xi_2,\xi_3$ fail to embed $(\mu_1,\mu_2,\mu_3)$. 
Modifying this example, we point out what we believe is a major challenge for defining an iterated Az\'{e}ma-Yor type embedding in the general case. 


In Figure \ref{fig:potentials_couterexample} we define measures via its potentials
\begin{align}
U\mu:\R \to \R, \quad U\mu(x):= -\int_{\R}{ \left| u-x \right| \mu(\dd u) }.
\end{align}
We refer to \cite[Proposition 2.3]{Obloj:04b} for some properties of $U\mu$.



\begin{figure}[htb]
\begin{center}
\includegraphics[scale=0.85]{plots/potentials_and_stopping_boundaries_plots_new/potential_plots_embedding_paper.pdf}  
\caption{Potentials of $\mu_1,\mu_2$, $\mu_3, \nu_2$ and $\nu_3$.}
\label{fig:potentials_couterexample}
\end{center} 
\end{figure}

 

\begin{figure}[htb]
\begin{center}
\includegraphics[scale=0.85]{plots/potentials_and_stopping_boundaries_plots_new/true_and_obtained_boundaries.pdf}  
\caption{The (unique) boundaries $b_1,b_2,b_3$ required for the embedding of $(\mu_1,\mu_2,\mu_3)$ and the stopping boundary $\xi_3$ obtained from \eqref{eq:definition_xi_n}.}
\label{fig:stopping_boundaries_couterexample}
\end{center} 
\end{figure}


%\begin{comment}

Observe that the embedding for $\left(\mu_1, \mu_2, \mu_3\right)$ is unique: We write $T_{a,b}$ for the exit time of $[a,b]$ and denote $T_{a,b} \circ \theta_\tau := \inf\left\{ t>\tau:B_t \not \in (a,b) \right\}$. Then the embedding $\left(\tau_1,\tau_2,\tau_3\right)$ can be written as
\begin{align}
\tau_1 = T_{-1,3}, \qquad \tau_2 =  T_{-2,0} \circ \theta_{\tau_1}, \qquad \tau_3 = T_{-2,3} \circ \theta_{\tau_2}.
\label{eq:unique_stopping_time_counterexample}
\end{align}

We obtain the same stopping boundaries $\xi_1,\xi_2$ as the method of \cite{Brown98themaximum},
\begin{align*}
\xi_1(y):= \begin{cases} 
-1 & \text{if $y \in [0,3)$,}   \\
y & \text{else,}
\end{cases}
\qquad \qquad \qquad
\xi_2(y):= \begin{cases} 
-3 & \text{if $y = 0$,}   \\
y & \text{else.}
\end{cases}
\end{align*}
This already shows that our embedding fails to embed $(\mu_1,\mu_2)$. 
The point we want to make now is that the optimization problem \eqref{eq:definition_xi_n} does not return the third (unique) stopping boundary which is required for the embedding of $(\mu_1,\mu_2,\mu_3)$.
Indeed, for sufficiently small $y>0$, in the region $\zeta<\min(\xi_1(y),\xi_2(y)) = -1$ we are looking at the minimization of $\zeta \mapsto \frac{c_3(\zeta)}{y-\zeta}$ which is attained by $\xi_3(y)=-3<-2$ since $\mu_3$ has an atom at $-3$. Consequently, there will be a positive probability to hit $-3$ after $\tau_2$.
This contradicts \eqref{eq:unique_stopping_time_counterexample}.

This example does not contradict our main result because Assumption $\ref{ass:unicity_minimizers}$(ii)(a) is not satisfied for $i=2$ and $y=0$, where $\zeta=-3$ minimizes the objective function but $c_2(0) = c_1(0)$ holds.

\tbd discontinuities not main problem, cf.   

\tbd note $\xi_n(y) = y$ possible and required to define embedding.

We note however that there exists an embedding which might be termed \enquote{iterated Az\'{e}ma-Yor type embedding} although this embedding does not satisfy the relations from Lemma \ref{lem:Key_Properties_of_the_Stopping_Rule}.
Consequently, one might conjecture that a modification of the optimization problem \eqref{eq:definition_xi_n} and a relaxation of Lemma \ref{lem:Key_Properties_of_the_Stopping_Rule} might fix this problem. 
We highlight an additional obstacle when attempting to do this. 

%\begin{figure}[ht]
%\includegraphics[scale=1]{plots/counterexample_embedding_paper.pdf}  
%\caption{Potentials of $\mu_1,\mu_2$ and $\mu_3$.}
%\label{fig:potentials_couterexample}
%\end{figure}

 
%\subsection{Discussion of Assumption \ref{ass:unicity_minimizers} and General Embedding}


To this end consider the measures $\mu_1, \nu_2,\nu_3$ defined via its potentials in Figure \ref{fig:potentials_couterexample}. 
In order to understand the problem in more detail, let us indicate how the \cite{Brown98themaximum} embedding for $\left(\mu_1,\nu_2\right)$ looks like. 
It reads
\begin{align*}
\tau_1^{\mathrm{BHR}} := \tau^{\mathrm{AY}}_1 = \tau_1, \qquad \qquad
\tau^{\mathrm{BHR}}_2:= \begin{cases} 
\tau^{\mathrm{BHR}}_1 & \text{if $B_{\tau^{\mathrm{BHR}}_1} \geq 0$,}   \\
\tau'_2 & \text{else,} 
\end{cases}
\end{align*}
where $\tau'_2$ is some stopping time embedding $\restr{\mu_1}{(-\infty,0)} = \mu_1(-\infty,0) \cdot \delta_{\left\{ -1 \right\}}$ into $\restr{\mu_2}{(-\infty,0)}$ without changing the maximum at time $\tau^{\mathrm{BHR}}_1$, i.e. 
\begin{align*}
\bar{B}_{\tau'_2} = \bar{B}_{\tau^{\mathrm{BHR}}_1}.
\end{align*} 
There are infinitely many such stopping times. 

As above, we note that our embedding fails to embed $\left(\mu_1,\nu_2\right)$, however we obtain the same stopping boundaries as \cite{Brown98themaximum}. The key problem we have for the third embedding is that
\begin{align}
\tau'_2 > \tau_3 \qquad \text{with positive probability for every $\tau'_2$.}
\end{align}
Hence, in general we are not able to performing a similar \enquote{correction} as the one corresponding to $\tau'_2$ and do our embedding on top of that.

In other words, when attempting to define the embedding $\tau_3$ for $\nu_3$ on top of the \cite{Brown98themaximum} embedding for $\left(\mu_1,\nu_2\right)$ the choice of $\tau'_2$ matters, both for the embedding and the distribution of the maximum $\bar{B}_{\tau_3}$.
This is the main reason why we believe that a genuinely new idea is needed to define the embedding in all generality.

We have talked about the strong association between $M_n$ and $\bar{M}_n$ which yields \enquote{extreme} properties for the process $M$. 
One feature of this can be seen by taking the limit to a continuum of marginals $\left( \mu_t \right)_{t \geq 0}$ (after defining an appropriate analogue of Assumption \ref{ass:unicity_minimizers}) which yields a process which has only positive jumps and in between these jumps it is either constant or decreasing.


To sum it up, our example shows that if Assumption \ref{ass:unicity_minimizers} does not hold the optimization problem \eqref{eq:definition_xi_n} might yield the wrong stopping boundary for the embedding. 
At the same time we have also seen in Example \ref{ex:MadanYor} that Assumption \ref{ass:unicity_minimizers} is too restrictive. 
It implies continuity of $\xi_2,\dots,\xi_n$ which is used in the proof of the embedding property. However, in the \enquote{increasing mean residual value} case, cf. \eqref{eq:IMRV}, the embedding can be easily shown by noting that a discontinuity of $\xi_i$ corresponds to a gap in support of $\mu_i$. From \eqref{eq:IMRV} it follows that no mass can be placed at this \enquote{jump interval} and so in principle our proof could be adapted to cover the \cite{MadanYor} case.
More generally, if one can make sure that the embedding property is satisfied at discontinuities of the stopping boundaries, Assumption \ref{ass:unicity_minimizers}(ii) could be relaxed slightly.

%\tbd In general, law of maximum $\leq$: Follows easily from pathwise inequality in \cite{Touzi_maxmax}. 


%\end{comment}

==> general_embedding_n_3.tex <==

\subsection{Sketch for General Embedding in the Case $n=3$ }
\label{subsec:general_embedding_n_3}

In the example of the measures $(\mu_1,\mu_2,\mu_3)$ from \eqref{eq:counterexample_mu_1}--\eqref{eq:counterexample_mu_3} the (unique) embedding could still be seen as a type of \enquote{iterated Az\'{e}ma-Yor type embedding} although it does not satisfy the relations from Lemma \ref{lem:Key_Properties_of_the_Stopping_Rule}.
Consequently, one might conjecture that a modification of the optimization problem \eqref{eq:definition_xi_n} and a relaxation of Lemma \ref{lem:Key_Properties_of_the_Stopping_Rule} might lead to a generally applicable embedding. We now explain in which sense this is true. Our aim is to outline new ideas and arguments which are needed. The technical details quickly become very involved and lengthy. In the sake of brevity, but also to better illustrate the main points, we restrict ourselves to a formal discussion and the case $n=3$.

In order to understand the problem in more detail, we need to recall from \cite{Brown98themaximum} how the embedding for $\mu_2$ looks like in general. 
It reads
\begin{align}
\tau^{\mathrm{BHR}}_2:= \begin{cases} 
\tau'_2 & \text{if $\xi_2^{-1} \neq \xi_1(\bar{B}_{\tau_1})$ and $\xi_1(\bar{B}_{\tau_1}) < \xi_2(\bar{B}_{\tau_1})$,}   \\
\tau_2 & \text{else,} 
\end{cases}
\label{eq:extensions_BHR_embedding}
\end{align}
where $\tau'_2$ is some stopping time with $\bar{B}_{\tau_2}=\bar{B}_{\tau_2'}$. Its  existence is established in \cite{Brown98themaximum} by showing that the relative parts of the mass which are further diffused have the same mass, mean and are in convex order. 
In general there will be infinitely many such stopping times $\tau'_2$. Although this is not true for $(\mu_1,\mu_2,\mu_3)$ in \eqref{eq:counterexample_mu_1}--\eqref{eq:counterexample_mu_3} because their embedding was unique, it is true for  measures $(\mu_1,\nu_2,\nu_3)$ which are defined via their potentials in Figure \ref{fig:potentials_couterexample}. 

Let $\xi_1$ and $\xi_2$ be defined as in \eqref{eq:definition_xi_n} and let $M_2 = B_{\tau_2}$.
Now our goal is to define an embedding $\tilde{\tau}_3$ for the third marginal on top of the \cite{Brown98themaximum} embedding in a situation as in $\left(\mu_1, \nu_2, \nu_3 \right)$. We still want to define our iterated Az\'{e}ma-Yor type embedding through a stopping rule based on some stopping boundary $\tilde{\xi}_3$ as a first exit time,
\begin{align}
\tilde{\tau}_3:= \begin{cases} 
\inf\left\{ t \geq \tau^{\mathrm{BHR}}_2 : B_t \leq \tilde{\xi	}_3(\bar{B}_t) \right\} & \text{if $B_{\tau^{\mathrm{BHR}}_2} > \tilde{\xi}_3(\bar{B}_{\tau^{\mathrm{BHR}}_2})$,}   \\
\tau^{\mathrm{BHR}}_2 & \text{else,} 
\end{cases}
\label{eq:extension_tau_3}
\end{align}
and prove that this is a valid embedding of $\mu_3$.
We observe that now the choice of $\tau'_2$ in the definition of $\tau^{\mathrm{BHR}}_2$ may matter both for the embedding and the distribution of the maximum $\bar{B}_{\tilde{\tau}_3}$. Similarly as in \cite{Brown98themaximum} we expect that this will be only possible if the procedure which produces $\tilde{\xi}_3$ yields a continuous $\tilde{\xi}_3$. Otherwise an additional step, producing a stopping time $\tau_3'\geq \tilde{\tau}_3$ would be required and further complicate the presentation.

With this, a more canonical approach in the context of Lemma \ref{lem:Key_Properties_of_the_Stopping_Rule} is to write
\begin{align}
\label{eq:book_keeping}
\PP \left[ \bar{M}_3 \geq y \right] &= \PP \left[ M_3 \geq \tilde{\xi}_3(y) \right] + \text{\enquote{error-term}},
\end{align}
which we formalize in \eqref{eq:extension_decomposition_of_maximum}.
As it will turn out, this \enquote{error-term} provides a suitable \enquote{book-keeping procedure} to keep track of the masses in the embedding. 
We proceed along the lines of the proof of our main result. For simplicity, we further assume that $\xi_2$ has only one discontinuity, i.e. $\Xi_{-}:=\xi_2(\underline{y}-)<\xi_2(\underline{y}+):=\Xi_{+}$ for some $\underline{y} \geq 0$ and we let $\bar{y}:=\xi_1^{-1}(\Xi_{+})$. This is not a restriction, as explained below.





\subsubsection{Redefining $\xi_3$ and $K_3$}

Define the following auxiliary terms,
\begin{alignat}{3}
&F(\zeta,y;\tau'_2) &&:= \indicator{\bar{M}_{1} \in [y,\bar{y}], y \geq \underline{y}}  \big( \zeta - M_2 \big)^+,\label{eq:aux_term} \\
&f^{\mathrm{iAY}}(\zeta,y;\tau'_2) &&:= \EE\left[ F(\zeta,y;\tau'_2) \right], \\
&G(\zeta,y;\tau'_2) &&:= \indicator{\bar{M}_{1} \in [y,\bar{y}, M_1 < M_2], y \geq \underline{y}}  \big( M_2 - \zeta \big)^+,\label{eq:aux_term_2} \\
&g^{\mathrm{iAY}}(\zeta,y;\tau'_2) &&:= \EE\left[ F(\zeta,y;\tau'_2) \right].
\end{alignat}
As the notation underlines, these quantities may depend on the additional choice of stopping time $\tau_2'$ between $\tau_2$ and $\tau_3$. Note that for $y \geq \underline{y}$,
\begin{align}
\frac{\partial f^{\mathrm{iAY}}}{\partial \zeta}(\zeta,y;\tau'_2) &= \PP\left[ \bar{M}_1 \in [y,\bar{y}], M_2 < \zeta \right], \label{eq:partial_derivative_f_x} %\\
%\frac{\partial^2 f^{\mathrm{iAY}}}{\partial \zeta \partial y}(\zeta,y;\tau'_2) &= -\frac{\PP\left[ \bar{M}_1 \in \dd y, M_2 < \zeta \right]}{\dd y}, \label{eq:partial_derivative_f_x_y}
\end{align}
and 
\begin{align}
\frac{\partial f^{\mathrm{iAY}}}{\partial y}(\zeta,y;\tau'_2) 
&= -\EE\left[ \frac{\indicator{\bar{M}_1 \in \dd y, M_2<\zeta}}{\dd y} \right] \zeta +  \EE\left[ \frac{\indicator{\bar{M}_1 \in \dd y, M_2<\zeta}}{\dd y} M_2 \right] \nonumber \\
&=-\Big(\zeta - \alpha(\zeta,y;\tau'_2)\Big)\frac{\PP\left[ \bar{M}_1 \in \dd y, M_2<\zeta \right]}{\dd y}
\label{eq:partial_derivative_f_y}
\end{align}
where
\begin{align}
\alpha(\zeta,y;\tau'_2) &:= \EE\left[ M_2 \big \vert \bar{M}_1 = y, M_2<\zeta \right], \\
\beta(\zeta,y;\tau'_2)  &:= \EE\left[ M_2 \big \vert \bar{M}_1 = y, M_2 \geq \zeta \right].
\end{align}
With these definitions we have by the properties of $\tau'_2$,
\begin{equation}
\begin{split} 
 & \alpha(\zeta,y;\tau'_2)\frac{\PP\left[ \bar{M}_1 \in \dd y, M_2<\zeta \right]}{\dd y} + \beta(\zeta,y;\tau'_2)\frac{\PP\left[ \bar{M}_1 \in \dd y, M_2 \geq \zeta \right]}{\dd y} \\
=& \xi_1(y) \frac{\PP\left[ \bar{M}_1 \in \dd y  \right]}{\dd y}.
\end{split}
\label{eq:relation_alpha_beta}
\end{equation}

We now redefine $\xi_3$ and $K_3$ from \eqref{eq:definition_xi_n} and \eqref{eq:definition_Kn}, respectively, and denote the new definition by $\tilde{\xi}_3$ and $\tilde{K}_3$. 
To this end, introduce the function
\begin{numcases}{\tilde{c}^3(\zeta,y):=}
c_3(\zeta)-f^{\mathrm{iAY}}(\zeta,y;\tau'_2)& \text{if $f^{\mathrm{iAY}}(\zeta,y;\tau'_2)>0$ and $\zeta<\Xi_+$, \qquad \quad}
\label{eq:redefintion_tilde_c_3_a} \\
c^3(\zeta,y)    & \text{else.}
\label{eq:redefintion_tilde_c_3_b}
\end{numcases} 
and, as before, let 
\begin{align}
\tilde{\xi}_3(y):=\argmin_{\zeta < y}\frac{\tilde{c}^3(\zeta,y)}{y-\zeta}
\end{align}
and 
\begin{align}\label{eq:def_tildeK3}
\tilde{K}_3(y):=\frac{\tilde{c}^3(\tilde{\xi}_3(y),y)}{y-\tilde{\xi}_3(y)}.
\end{align}
It is clear that a discontinuity of $\xi_2$ results in a local perturbation of $c^3$ into $\tilde c^3$ and in consequence of $\xi_3$ into $\tilde \xi_3$. If $\xi_2$ has multiple discontinuities the construction above applies to each of them giving a global definition of $\tilde c^3$. Then $\tilde K_3$ and $\tilde \xi_3$ are defined as above.

In the redefined domain, i.e.\ if $f^{\mathrm{iAY}}(\zeta,y;\tau'_2)>0$ and $\zeta<\Xi_+$, the first order condition for optimality of $\tilde{\xi}_3(y)$ reads
\begin{align}
\tilde{K}_3(y) +  c'_3(\tilde{\xi}_3(y)) - \frac{\partial f^{\mathrm{iAY}}}{\partial \zeta}(\tilde{\xi}_3(y),y;\tau'_2)  = 0.
\label{eq:optimality_tilde_xi}
\end{align}
We stress that now the quantities $\tilde{\xi}_3$ and $\tilde{K}_3$ may depend on $\tau'_2$.


\subsubsection{Monotonicity of $\tilde{\xi}_3$}


\begin{comment}

The term $f^{\mathrm{iAY}}(\zeta,y;\tau'_2)$ has the interpretation of a penalty term. 
As seen in Lemma \ref{lem:Contributions to the Maximum}, if Assumption \ref{ass:unicity_minimizers}(ii) is in place then $\tau'_2=\tau_2$, $\tilde{\xi}_3(y) = \xi_3(y)$ and the term $\frac{\partial f^{\mathrm{iAY}}}{\partial \zeta}(\tilde{\xi}_3(y),y;\tau'_2)$ takes the convenient form of 
\begin{align*}
\PP\left[ M_{\jmath_3(y)} \geq \xi_3(y) \right] - \PP\left[ \bar{M}_{\jmath_3(y)} \geq y \right]
\end{align*}
and we are back in the setting of Sections \ref{sec:Main Assumption and Definitions} and \ref{sec:iAY}.

\tbd In general, one can check that $c^n(\xi_3(y),y)-\tilde{c}^n(\tilde{\xi}_3(y),y) \geq 0$ and therefore $f^{\mathrm{iAY}}(\tilde{\xi}_3(y),y;\tau'_2)$ is a stronger penalty.

 
\end{comment}
 
 
 
Our goal is to find a condition which ensures that $\tilde{\xi}_3$ will be non-decreasing. 
To this end we will use the (formal) first and second order conditions for optimality of $\tilde{\xi}_3(y)$.

 
We have
\begin{align}
\frac{\partial^2 f^{\mathrm{iAY}}}{\partial \zeta \partial y}(\zeta,y;\tau'_2) &= -\frac{\PP\left[ \bar{M}_1 \in \dd y, M_2 < \zeta \right]}{\dd y}. \label{eq:partial_derivative_f_x_y}
\end{align} 
 
Recalling the first order condition from \eqref{eq:optimality_tilde_xi},
\begin{align}
\tilde{K}_3(y) +  c'_3(\tilde{\xi}_3(y)) - \frac{\partial f^{\mathrm{iAY}}}{\partial \zeta}(\tilde{\xi}_3(y),y;\tau'_2)  = 0
\label{eq:optimality_tilde_xi_recall}
\end{align} 
and then the second order condition reads
\begin{align}
c''_3(\tilde{\xi}_3(y)) - \frac{\partial^2 f^{\mathrm{iAY}}}{\partial \zeta^2}(\tilde{\xi}_3(y),y;\tau'_2) \geq 0.
\label{eq:seond_order_condition_optimality}
\end{align}



\begin{comment}


Using the fact that $\tilde{K}_3 \geq 0$, we rearrange \eqref{eq:optimality_tilde_xi} to 
\begin{align*}
\frac{c_3(\tilde{\xi}_3(y))-f^{\mathrm{iAY}}(\tilde{\xi}_3(y),y;\tau'_2)}{-c'(\tilde{\xi}_3(y))+\frac{\partial f^{\mathrm{iAY}}}{\partial \zeta}(\tilde{\xi}_3(y),y;\tau'_2)} = y-\tilde{\xi}_3(y) \geq 0
\end{align*}
from which we conclude from the fact that the denominator equals $\tilde{K}_3 \geq 0$ (by \eqref{eq:optimality_tilde_xi}), that
\begin{align}
c_3(\tilde{\xi}_3(y))-f^{\mathrm{iAY}}(\tilde{\xi}_3(y),y;\tau'_2) \geq 0.
\end{align}


\end{comment}

Now, differentiating \eqref{eq:optimality_tilde_xi} in $y$ yields
\begin{align*}
\tilde{K}'_3(y) + c''_3(\tilde{\xi}_3(y)) \tilde{\xi}'_3(y) - \frac{\partial^2 f^{\mathrm{iAY}}}{\partial \zeta^2}(\tilde{\xi}_3(y),y;\tau'_2) \tilde{\xi}'_3(y) - \frac{\partial^2 f^{\mathrm{iAY}}}{\partial \zeta \partial y}(\tilde{\xi}_3(y),y;\tau'_2) = 0 
\end{align*}
or equivalently,
\begin{align*}
 \tilde{\xi}'_3(y)  \underbrace{ \left( c''_3(\tilde{\xi}_3(y))  - \frac{\partial^2 f^{\mathrm{iAY}}}{\partial \zeta^2}(\tilde{\xi}_3(y),y;\tau'_2) \right) }_{\geq 0 \text{ by \eqref{eq:seond_order_condition_optimality}}}   = - \tilde{K}'_3(y) + \frac{\partial^2 f^{\mathrm{iAY}}}{\partial \zeta \partial y}(\tilde{\xi}_3(y),y;\tau'_2)
\end{align*}

In order to formally infer
\begin{align}
\tilde{\xi}'_3(y) \geq 0
\end{align}
we require
\begin{align}
- \tilde{K}'_3(y) + \frac{\partial^2 f^{\mathrm{iAY}}}{\partial \zeta \partial y}(\tilde{\xi}_3(y),y;\tau'_2) \geq 0.
\label{eq:condition_monotonicity_tilde_xi}
\end{align}

{\sc We still have to establish the validity of \eqref{eq:condition_monotonicity_tilde_xi}!!!\\
In the following we assume \eqref{eq:condition_monotonicity_tilde_xi} to hold and hence that $\tilde \xi_3$ is non-decreasing.}


\subsubsection{Embedding Property}

In the following we assume that $\zeta$ and $y$ are such that $f^{\mathrm{iAY}}(\zeta,y;\tau'_2)>0$ and $\zeta<\Xi_+$. Otherwise $\tilde c^3 = c^3$ and the arguments from Sections \ref{sec:Main Assumption and Definitions} and \ref{sec:iAY} apply.
 
By definition of the embedding in \eqref{eq:extension_tau_3}, and since $\tilde{\xi}_3$ is non-decreasing, we have
\begin{alignat}{3}
\PP \left[ \bar{M}_3 \geq y \right] &= \hspace{3mm} &&\PP \left[ M_3 \geq \tilde{\xi}_3(y) \right] + \PP\left[ \bar{M}_3 \geq y, M_3 < \tilde{\xi}_3(y) \right] \nonumber \\
									 &= &&\PP \left[ M_3 \geq \tilde{\xi}_3(y) \right] + \PP\left[ \bar{M}_1 \geq y, M_2 < \tilde{\xi}_3(y) \right] \nonumber \\
									 &= &&\PP \left[ M_3 \geq \tilde{\xi}_3(y) \right] + \PP\left[ \bar{M}_1 \in [y,\bar{y}], M_2 < \tilde{\xi}_3(y) \right] \nonumber \\
									 &\stackrel{\mathclap{\eqref{eq:partial_derivative_f_x}}}{=} &&\PP \left[ M_3 \geq \tilde{\xi}_3(y) \right] + \frac{\partial f^{\mathrm{iAY}}}{\partial \zeta}(\tilde{\xi}_3(y),y;\tau'_2).
									 \label{eq:extension_decomposition_of_maximum}
\end{alignat}

%We compute further
%\begin{alignat}{3}
%\PP \left[ \bar{M}_3 \geq y \right] = & &&\int_0^{\underline{y}} \PP\left[ \bar{M}_1 \in \dd s\right] \frac{ \left( \xi_1(s) - \underline{\xi}_1(s) \right)^+}{s-\underline{\xi}_1(s)} \exp\left(- \int_{s}^{y} \frac{\dd r}{r-\underline{\xi}_1(r)} \right) \nonumber \\
%									   &+&&\int_{\underline{y}}^y  p(\tilde{\xi}_3(s),s;\tau'_2) \exp\left(- \int_{s}^{y} \frac{\dd r}{r-\tilde{\xi}_3(r)} \right) \nonumber \\
%									   &+&&\PP \left[ \bar{M}_1 \geq y \right]
%									   \nonumber
%\end{alignat}
%for some $\underline{\xi}_1$ such that $\underline{\xi}_1(y) = \tilde{\xi}_3(y)$ and where
Note that
\begin{align}
&\restr{\frac{\partial \PP \left[ \bar{M}_1 \in [\underline{y},y), \bar{M}_3 \geq m \right]}{\partial y}}{m=y} = p(\tilde{\xi}_3(y),y;\tau'_2) := \label{eq:definition_p_probability} \\ 
&\frac{ \PP\left[ M_2>\tilde{\xi}_3(y), \bar{M}_1 \in \dd y \right]}{\dd y} \cdot \PP \left[ H_y \circ \theta_{\tau'_2} < H_{\tilde{\xi}_3(y)} \circ \theta_{\tau'_2} \big\vert M_2>\tilde{\xi}_3(y), \bar{M}_1 = y \right] %\\
								%&= \frac{ \PP \left[ \bar{M}_1 \in \dd s, M_2>\tilde{\xi}_3(s), H_s \circ \theta_{\tau'_2} < H_{\tilde{\xi}_3(s)} \circ \theta_{\tau'_2} \right]}{\dd s}.
\nonumber
\end{align}
where as above $H_x:=\inf\left\{ t \geq 0:B_t=x \right\}$. Combining this with the obvious decomposition
\begin{align*}
\PP \left[ \bar{M}_3 \geq y \right] = \PP \left[ \bar{M}_1 < \underline{y}, M_3 \geq y \right] + \PP \left[ \bar{M}_1 \in [\underline{y},y), \bar{M}_3 \geq y \right] + \PP \left[ \bar{M}_1 \geq y \right]
%\label{eq:extension_trivial_decomposition}
\end{align*}
and similar excursion theoretical arguments as in the proof of Lemma \ref{lem:ODE_for_the_Maximum}, we obtain
\begin{align}
\frac{\partial}{\partial y}\PP \left[ \bar{M}_3 \geq y \right] 
&=  -\frac{\PP \left[ \bar{M}_3 \geq y \right] - \PP\left[ \bar{M}_1 \geq y \right] }{y-\tilde{\xi}_3(y)} +   p(\tilde{\xi}_3(y),y;\tau'_2) + \frac{\partial \PP\left[ \bar{M}_1 \geq y \right]}{\partial y}  \nonumber \\
&\stackrel{\mathclap{\eqref{eq:ODE_law_maximum}}}{=} -\frac{\PP \left[ \bar{M}_3 \geq y \right] }{y-\tilde{\xi}_3(y)} +   p(\tilde{\xi}_3(y),y;\tau'_2) -  \frac{\tilde{\xi}_3(y)-\xi_1(y)}{y-\tilde{\xi}_3(y)} \frac{\partial \PP\left[ \bar{M}_1 \geq y \right]}{\partial y}.
\end{align}

By similar calculations as in \eqref{eq:ODE_K_N_proof} below we have
\begin{alignat*}{3}
\tilde{K}'_3(y) \stackrel{\mathclap{\eqref{eq:optimality_tilde_xi}}}{=} &-&& \frac{\tilde{K}_3(y)}{y-\tilde{\xi}_3(y)} - \frac{\frac{\partial f^{\mathrm{iAY}}}{\partial y}(\tilde{\xi}_3(y),y;\tau'_2)}{y-\tilde{\xi}_3(y)} \nonumber \\
				\stackrel{\mathclap{\eqref{eq:partial_derivative_f_y}}}{=} & - && \frac{\tilde{K}_3(y)}{y-\tilde{\xi}_3(y)} + \frac{ \tilde{\xi}_3(y) - \alpha(\tilde{\xi}_3(y),y) }{y-\tilde{\xi}_3(y)} \frac{\PP\left[ \bar{M}_1 \in \dd y, M_2<\tilde{\xi}_3(y) \right]}{\dd y} \nonumber \\
				\stackrel{\mathclap{\eqref{eq:relation_alpha_beta}}}{=} &-&& \frac{\tilde{K}_3(y)}{y-\tilde{\xi}_3(y)} + \frac{ \tilde{\xi}_3(y) - \xi_1(y) }{y-\tilde{\xi}_3(y)}\frac{\PP\left[ \bar{M}_1 \in \dd y  \right]}{\dd y} \nonumber \\
				&+&& \frac{ \beta(\tilde{\xi}_3(y), y) - \tilde{\xi}_3(y) }{y-\tilde{\xi}_3(y)} \frac{\PP\left[ \bar{M}_1 \in \dd y, M_2 \geq \tilde{\xi}_3(y) \right]}{\dd y} \nonumber \\
				\stackrel{\mathclap{\eqref{eq:definition_p_probability}}}{=} &-&& \frac{\tilde{K}_3(y)}{y-\tilde{\xi}_3(y)} - \frac{ \tilde{\xi}_3(y) - \xi_1(y) }{y-\tilde{\xi}_3(y)} \frac{\partial \PP\left[ \bar{M}_1 \geq y  \right]}{\partial y} + p(\tilde{\xi}_3(y),y;\tau'_2). 
\end{alignat*}

Consequently, as in Proposition \ref{prop:Maximizing the Maximum}, for all $y$,
\begin{align}
\tilde{K}_3(y) = \PP\left[ \bar{M}_3 \geq y \right]
\label{eq:extension_maximum_identification}
\end{align}
and then, by \eqref{eq:optimality_tilde_xi} and \eqref{eq:extension_decomposition_of_maximum},
\begin{align*}
-c'_3(\tilde{\xi}_3(y)) = \PP\left[ M_3 \geq \tilde{\xi}_3(y) \right]
%\label{eq:extension_embedding}
\end{align*}
which is the desired embedding property.
%If $\tilde{\xi}_3$ happens to be discontinuous, then we cannot guarantee the embedding property for $\mu_3$. However, we expect that similar arguments as those in \cite[Section 3.5]{Brown98themaximum} will yield a stopping time $\tau'_3$ which does the job for the jump-intervals of $\tilde{\xi}_3$.
%We do not pursue these matters here. 

The above construction hinged on the appropriate choice of the auxiliary term $F$ in \eqref{eq:aux_term} whose expectation, as follows from  \eqref{eq:redefintion_tilde_c_3_a}, \eqref{eq:def_tildeK3} and \eqref{eq:extension_maximum_identification}, allows for the error book keeping, as suggested in \eqref{eq:book_keeping}. We identified the correct $F$ by analysing the ``error terms" which cause strict inequality for $(B_u:u\leq \tau_2')$ in the pathwise inequality (4.1) in \cite{Touzi_maxmax}. This is natural since this inequality is used to prove optimality of our embedding. It gives an upper bound but fails to be sharp if condition (ii) in Assumption \ref{ass:unicity_minimizers} does not hold. In order to recover sharp bound one has to look at the error terms causing strict inequality when Assumption \ref{ass:unicity_minimizers} fails. The same principle applies for $n>3$. However then interactions between discontinuities of boundaries $\xi_2,\tilde \xi_3$ etc come into play and the relevant terms become hugely involved. The construction would become so technical and implicit that we decided to stop at this point.



==> hobson_klimmek.tex <==

\section{\cite{Hobson11} in $n$-Marginal Case} 

What are building blocks?

==> necessary_and_sufficient_condition_under_hobson.tex <==


\subsection{Necessary and Sufficient Condition under Hobson Assumption}

\subsubsection{$n=2$}

\begin{Proposition}
\label{prop:charterization_n_2}
Let $n=2$ and assume that 
\begin{itemize} 
	\item[(a)] Assumption \ref{ass:unicity_minimizers}(i) holds,	
	\item[(b)] $ x \mapsto c_2(x) - c_1(x) $ is concave on $(x_l,x_r)$ and convex on $(-\infty,x_l]$ and $[x_r,\infty)$,
	\item[(c)] $c_1<c_2$,
	\item[(d)] $b_i$ is strictly increasing.
\end{itemize}

Then Assumption \ref{ass:unicity_minimizers}(ii) is equivalent to the following:
if $b^{-1}_2(y) < b^{-1}_1(y)$ then for all $\beta$ such that $ b_1^{-1}(y) \leq \beta <y$ we have
\begin{align}
\bar{\mu}_2^{\mathrm{HL}}(y) - \bar{\mu}_1^{\mathrm{HL}}(y) < \frac{c_2(\beta) - c_1(\beta)}{y-\beta}.
\label{eq:charterization_n_2}
\end{align}
\end{Proposition}
\begin{proof}
We prove necessity of \eqref{eq:charterization_n_2}. 
If we can find $y$ and $\beta$ such that 
\begin{align*}
\bar{\mu}_2^{\mathrm{HL}}(y) - \bar{\mu}_1^{\mathrm{HL}}(y) = \frac{c_2(\beta) - c_1(\beta)}{y-\beta}
\end{align*}
then we must also have
\begin{align*}
c'_2( b_2^{-1}(y) ) = c'_2(\beta) - c'_1(\beta) - \bar{\mu}_1^{\mathrm{HL}}(y).
\end{align*}
Together with
\begin{align*}
\frac{ c^2(b_2^{-1}(y),y)}{y - b_2^{-1}(y) } = \frac{c^2(\beta,y)}{y-\beta}
\end{align*}
this yields that Assumption \ref{ass:unicity_minimizers}(ii) is violated.

Now we prove sufficiency.
To this end, assume that Assumption \ref{ass:unicity_minimizers}(ii) is violated, i.e. there are $\alpha < \beta<y$ such that
\begin{align*}
\frac{ c^2(\alpha,y)}{y - \alpha } = \frac{c^2(\beta,y)}{y-\beta}
\end{align*}
and 
\begin{align}
\frac{\partial c^2}{\partial x}(\alpha,y) = \frac{\partial c^2}{\partial x}(\beta,y).
\label{eq:suff_proof_optimality_n_2}
\end{align}
We need to show that $\alpha = b_2^{-1}(y) < b_1^{-1}(y) \leq \beta$.

If $\alpha < b_1^{-1}(y)$ then by assumption $\alpha = b_2^{-1}(y)$. By \eqref{eq:suff_proof_optimality_n_2} and (b) it is not possible that $\alpha \geq b_1^{-1}(y)$ (there are two points where $c_2-c_1$ have the same slope but then at these points the second derivatives have different signs). Similarly, by \eqref{eq:suff_proof_optimality_n_2} and (d) it is not possible that $\beta < b_1^{-1}(y)$.
\end{proof}

Proposition \ref{prop:charterization_n_2} states that under the Hobson assumption (b) there can only be jumps of $\xi_2$ across $\xi_1$. 
We capture them by \eqref{eq:charterization_n_2}.


\subsubsection{$n=3$}


==> numerical_verification.tex <==
 
\section{Numerical Example}

\subsection{Strictly Increasing Boundaries}

\tbd Check distribution of $\bar{M}^{\star}_n$.


%\subsection{Example: Four Given Stopping Boundaries}
%\subsubsection{Stopping Boundaries and Optimization Problems}

We assume that the underlying stock price process $M$ is generated by an iterated Az\'{e}ma-Yor embedding based on some fixed stopping boundaries $\xi_1,\dots,\xi_4$.
These stopping boundaries are displayed in Figure \ref{fig:computed_boundaries_boundary_example}.

We would like to illustrate the laws $\mu_1,\dots,\mu_4$ and the laws for the maximum, $K^1,\dots,K^4$, corresponding to the iterated Az\'{e}ma-Yor process based on the stopping boundaries $\xi_1,\dots,\xi_4$. 

Approaching this task numerically, in the first step we obtain an estimate $\hat{c}_1,\dots,\hat{c}_4,$ for the call prices $\hat{c}_1,\dots,c_n,$ for this process.
These call prices are shown in terms of its Black-Scholes implied-volatility smile in Figure \eqref{fig:implied_volatilities_boundary_example}. 

In the second step, we compute the stopping boundaries $\hat{\xi}_1, \dots,\hat{\xi}_4$ and the tail-distributions of the maxima, $\hat{K}^1, \dots, \hat{K}^4$, based on $\hat{c}_1,\dots,c_n$, cf. Definition \ref{def:indices}. 
The computed tail-distributions of the maxima, $\hat{K}^1, \dots, \hat{K}^4$, are displayed in Figure \ref{fig:implied_volatilities_boundary_example}.




\begin{figure}
	\centering		\includegraphics{plots/boundary_example/4marginals/computed_boundaries_boundary_example.pdf}
	\label{fig:computed_boundaries_boundary_example}
	\caption{Stopping boundaries $\xi_1,\dots,\xi_4$ used for the underlying iterated Az\'{e}ma-Yor process.} 
\end{figure}



%\subsubsection{Call Prices}

\begin{figure}[ht]
\label{fig:implied_volatilities_boundary_example}
\vspace{-2.5cm}
\mbox{
%\hspace{-20mm}
\subfigure{\includegraphics[width=0.95\textwidth]{plots/boundary_example/4marginals/implied_volatilities_boundary_example.pdf}}
}
\label{fig:calls_boundary_example}
\mbox{%\vspace{-2cm}
%\hspace{-20mm}
\subfigure{\includegraphics[width=0.95\textwidth]{plots/boundary_example/4marginals/relation_optimization_problems_boundary_example.pdf}}
}
\caption{Smiles and distribution of the maximum.} 
\end{figure}






\subsection{Jump Example}

\begin{figure}
	\centering
		\includegraphics[ angle=270, width=1.1\textwidth]{plots/jump_example/jump_example.pdf}
	\caption{Defined boundaries.}
	\label{fig:jump_example}
\end{figure}

\begin{figure}
	\centering
		\includegraphics[ angle=270, width=1.1\textwidth]{plots/jump_example/jump_example_impl_vols.pdf}
	\caption{Implied volatilities.}
	\label{fig:jump_example_impl_vols}
\end{figure}

\begin{figure}
	\centering
		\includegraphics[ angle=270, width=1.1\textwidth]{plots/jump_example/computed_boundaries_jump_example.pdf}
	\caption{Computed boundaries.}
	\label{fig:computed_boundaries_jump_example}
\end{figure}


\begin{figure}
	\centering
		\includegraphics[ angle=270, width=1.1\textwidth]{plots/jump_example/relation_optimization_problems_jump_example.pdf}
	\caption{Global optimization problem vs. sequence of optimization problems.}
	\label{fig:relation_optimization_problems_jump_example}
\end{figure}

\begin{figure}
	\centering
		\includegraphics[ angle=270, width=1.1\textwidth]{plots/jump_example/comparison_boundaries_jump_example.pdf}
	\caption{Minimizers from global minimization.}
	\label{fig:comparison_boundaries_jump_example}
\end{figure}

















\begin{comment}
\begin{figure}[ht]
\vspace{-2.5cm}
\mbox{
%\hspace{-20mm}
\subfigure{\includegraphics[width=1.0\textwidth]{plots/boundary_example/4marginals/computed_boundaries_boundary_example.pdf}}
}
\label{fig:computed_boundaries_boundary_example}
\mbox{%\vspace{-2cm}
%\hspace{-20mm}
\subfigure{\includegraphics[width=1.0\textwidth]{plots/boundary_example/4marginals/relation_optimization_problems_boundary_example.pdf}}
}
\label{fig:relation_optimization_problems_boundary_example}
\caption{Example: Given Stopping Boundaries. The underlying process itself is obtained from iterating the Azema-Yor embedding using the stopping boundaries $\xi_1,\dots,\xi_4$. Comparison of Global Optimization Problem with the value of $K^4$.} 
\end{figure}
\end{comment}


\begin{comment}
\subsection{Example: Black-Scholes, IMRV}

We use
\begin{equation}
\begin{split}
&c_i=\mathrm{BS}(S_0=100, \sigma_i, r=0, T=1), \quad \text{where } \\
&\sigma_1=\frac{6}{30}=0.2, \quad  \sigma_2=\frac{7}{30}, \quad \sigma_3=\frac{8}{30}, \quad \sigma_4=\frac{9}{30}=0.3.
\end{split}
\end{equation}

\begin{figure}[ht]
\vspace{-2.5cm}
\mbox{
%\hspace{-10mm}
\subfigure{\includegraphics[width=1.0\textwidth]{plots/BS_example/boundaries_in_BS_example.pdf}}}
\caption{Computed and true stopping boundaries in the Black-Scholes/ IMRV example.} 
\end{figure}

\end{comment}

\begin{comment}

\subsection{Example: Three Given Stopping Boundaries}
%\subsubsection{Stopping Boundaries and Optimization Problems}

We assume that the underlying stock price process $M$ is generated by an iterated Azema-Yor embedding based on some fixed $\xi_1,\xi_2,\xi_3$. 
In the first step we compute the corresponding call prices for this process $M$, cf. Figure \ref{fig:computed_boundaries_boundary_example}.   

\begin{figure}[ht]
\vspace{-2.5cm}
\mbox{
%\hspace{-20mm}
\subfigure{\includegraphics[width=1.0\textwidth]{plots/boundary_example/3marginals/computed_boundaries_boundary_example.pdf}}
}
\label{fig:computed_boundaries_boundary_example}
\mbox{%\vspace{-2cm}
%\hspace{-20mm}
\subfigure{\includegraphics[width=1.0\textwidth]{plots/boundary_example/3marginals/relation_optimization_problems_boundary_example.pdf}}
}
\label{fig:relation_optimization_problems_boundary_example}
\caption{Example: Given Stopping Boundaries. The underlying process itself is obtained from iterating the Azema-Yor embedding using the stopping boundaries $\xi_1,\xi_2,\xi_3$. Comparison of Global Optimization Problem with the value of $K^n$.} 
\end{figure}

%\subsubsection{Call Prices}

\begin{figure}[ht]
\vspace{-2.5cm}
\mbox{
%\hspace{-20mm}
\subfigure{\includegraphics[width=1.0\textwidth]{plots/boundary_example/3marginals/calls_boundary_example.pdf}}
}
\label{fig:calls_boundary_example}
\mbox{%\vspace{-2cm}
%\hspace{-20mm}
\subfigure{\includegraphics[width=1.0\textwidth]{plots/boundary_example/3marginals/implied_volatilities_boundary_example.pdf}}
}
\label{fig:implied_volatilities_boundary_example}
\caption{Example: Given Stopping Boundaries. Call prices and implied volatilities.} 
\end{figure}

\end{comment}



\begin{comment} 


\subsection{Example: Given Densities}

\tbd Define $\mu_i$ through densities $f_i$ such that the associated sequence of barycenter functions is not increasing.



\subsection{Example: Given Smiles}

\subsubsection{Stopping Boundaries and Optimization Problems}

\begin{figure}[ht]
\vspace{-2.5cm}
\mbox{
%\hspace{-20mm}
\subfigure{\includegraphics[width=1.0\textwidth]{plots/smiles_example/plot_boundaries_from_defined_smiles.pdf}}}
\mbox{%\vspace{-2cm}
%\hspace{-20mm}
\subfigure{\includegraphics[width=1.0\textwidth]{plots/smiles_example/relation_optimization_problems_smile_example.pdf}}}
\caption{Example: Given Smiles. } 
\end{figure}

\end{comment}

 






 



==> optimality_extensions.tex <==
\subsection{Optimality}

\textbf{Step 1: Reduction to Class of Iterated \AY Embeddings.}
\tbd Enough to look at iterated \AY embeddings at time $2$: inherited maximum largest,  can embed optimal \enquote{increment} on top of BHR (use path-swapping arguments).

\textbf{Step 2: Monotone boundary for time $3$.}
\tbd given a fixed BHR at time $2$ it is optimal to use some monotone boundary $\tilde{\xi}$ for $\mu_3$.



\textbf{Step 3: Choice of Optimal $\tau'_2$.}
Parametrize $\tau'_2$ by two exit boundaries $\gamma_l$ and $\gamma_r$.
Choose optimal $\tau'_2$:
\begin{align}
\sup_{\tau'_2} \left\{ -\E{ \pp{ M^{(\tau'_2)}_2 - \zeta } \indicator{\bar{M}_1 \geq y} } + (y-\zeta) K_1(y) \right\}
\end{align}
i.e. it is sufficient to solve
\begin{align}
\inf_{\tau'_2} \E{ \pp{ M^{(\tau'_2)}_2 - \zeta } \indicator{\bar{M}_1 \geq y} }. 
\end{align}

\tbd intuition: choose smallest $\gamma_l$ and/or maximize for each $y$ the quantity $\gamma_r(y) - \xi_1(y)$ subject to $y \mapsto \gamma_r(y) - \xi_1(y)$ being non-decreasing.

\tbd intuition: \enquote{maximal number of second chances}

==> optimization_problem_and_optimal_boundaries.tex <==


\section{Optimization Problem and Optimal Boundaries}

 
Assume that $\xi_1(y),\dots,\xi_{n-1}(y)$ and $K_y^{1},\dots,K_y^{n-1}$ are already defined. 

\begin{Definition}
\label{def:indices}
For convenience set $K^0_y \equiv 0$, $C_0\equiv 0$, $c_0\equiv 0$,  $\xi_{0}\equiv -\infty$, and  $\zeta_{n+1}(y)=y = \xi_{n+1}(y)$ for $y>0$.

For $y>0$ define
\begin{equation}
\begin{split}
&\imath_n(\cdot;y): (-\infty,y] \to \left\{ 0,1,\dots,n-1 \right\}, \\ 
&\imath_n(\zeta;y) := \max \left\{k \in \{ 0,1,\dots,n-1 \}: \xi_{k}(y) < \zeta \right\},
\end{split}
\end{equation} 
\begin{align}
\xi_n(y) \in \argmin_{\zeta < y} \left\{  \frac{c_n(\zeta)}{y-\zeta} - \left[ \frac{c_{\imath_n(\zeta;y)}(\zeta)}{y-\zeta} - K^{\imath_n(\zeta;y)}_y \right]   \right\},
\label{eq:definition_xi_n}
\end{align}
In addition define for $l=n-1,\dots, 1$, $y>0$
\begin{align}
\jmath_n(y) &:= \jmath(y) := \imath_n(\xi_n(y);y), \\
\jmath_l(y) &:= \max \left\{k \in \{ 0,1,\dots,\jmath_{l+1}(y)-1 \}: \xi_{k}(y) < \xi_{\jmath_{l+1}(y)}(y) \right\} ,
\label{eq:def_ordered_indices}
\end{align} 
and
\begin{align}
K_n(y):=\frac{1}{y-\xi_n(y)} \left\{ \vphantom{\frac{1}{y-\xi_n(y)}} c_n(\xi_n(y)) - \left[ c_{\jmath(y)}(\xi_n(y)) - (y-\xi_n(y)) K^{\jmath(y)}_y \right] \right\}.
\label{eq:definition_Kn}
\end{align}
\end{Definition}

\begin{Note}
All previously defined $\xi_1,\dots,\xi_{n-1}$ remain unchanged. $\xi_n$ is defined relative to $\xi_1,\dots,\xi_{n-1}$. In particular we do not need a backward substitution to define these quantities.
\end{Note}

\tbd $\xi_n$ right-continuous?

\tbd $K^n$ is continuous.

Note that from the definition of $\xi_n$, $\imath_n(\cdot;y)$ and $\jmath$ it follows that if $ \zeta \mapsto \frac{c_n(\zeta)}{y-\zeta} - \left[ \frac{c_{\imath_n(\zeta;y)}(\zeta)}{y-\zeta} - K^{\imath_n(\zeta;y)}_y \right]   $ is differentiable at $\xi_n(y)$, then
\begin{align}
\frac{1}{y-\xi_n(y)} K_n(y) + \frac{1}{y-\xi_n(y)} \left( \vphantom{\frac{1}{y-\xi_n(y)}} c'_n(\xi_n(y)) - c'_{\jmath(y)}(\xi_n(y)) - K_y^{\jmath(y)} \right) = 0.
\label{eq:optimality_xi}
\end{align}

\tbd Compare \eqref{eq:optimality_xi} with \eqref{eq:decomposing_the _maximum}.

\tbd In the other case, do we have 
\begin{align}
\xi'_n(y)=0?
\label{eq:constant_xi_n}
\end{align}

\begin{Lemma}
The optimization problem \eqref{eq:definition_xi_n} has a solution.

In addition, for all i=1,\dots,n, the mapping
\begin{align}
\R_+ \to \R, \quad y \mapsto \xi_i(y) 
\end{align}
is non-decreasing. 
\end{Lemma}
\begin{proof}
Existence of a solution to \eqref{eq:definition_xi_n} follows from the continuity of the objective function $\zeta \mapsto \frac{c_n(\zeta)}{y-\zeta} - \left[ \frac{c_{\imath_n(\zeta;y)}(\zeta)}{y-\zeta} - K^{\imath_n(\zeta;y)}_y \right] $.

We adapt the proof of \cite[Lemma 4.6]{Touzi_maxmax}. 

Let $I_0,I_1,\dots,I_l$ and $0=k_0<k_1<k_2<\dots<k_l$, $I_0=(-\infty,\xi_{k_1}], I_l=(\xi_{k_l},y]$ be such that $\dot{ \bigcup }_{j \leq l} I_j = (-\infty,y)$ and $\restr{\imath_n(\cdot;y)}{I_j} = k_j$. 
With this notation we can rewrite the optimization problem for $\xi_n$ as 
\begin{align*}
\xi_n(y) \in \argmin 					   \left\{ \vphantom{\min_{\zeta \in (-\infty,\xi_{k_1})} \frac{c_n(\zeta)}{y-\zeta} - \left[ \frac{c_{k_0}(\zeta)}{y-\zeta} - K^{k_0}_y \right] } \right. 							& \min_{\zeta \in (-\infty,\xi_{k_1})} \frac{c_n(\zeta)}{y-\zeta} ,  \\  
																				 & \min_{\zeta \in [\xi_{k_1},\xi_{k_2})} \frac{c_n(\zeta)}{y-\zeta} - \left[ \frac{c_{k_1}(\zeta)}{y-\zeta} - K^{k_1}_y \right],	\\
																				 & \quad \quad \dots	 \\
																				 & \left. \min_{\zeta \in [\xi_{k_{l}},y)} \frac{c_n(\zeta)}{y-\zeta} - \left[ \frac{c_{k_{l}}(\zeta)}{y-\zeta} - K^{k_{l}}_y \right] \right\}.
\end{align*}
Denote by $\mathcal{H}_{\min}^{j}$ the set of interior minimizers of $\zeta \mapsto \frac{c_n(\zeta)}{y-\zeta} - \left[ \frac{c_{k_j}(\zeta)}{y-\zeta} - K^{k_j}_y \right]$ on $[\xi_{k_l}, \xi_{k_{l+1}}]$.
The first order condition for optimality is 
\begin{align}
y=\frac{ \int_{\zeta}^{\infty}{u \mu_n(\dd u)} - \int_{\zeta}^{\infty}{u \mu_{k_l}(\dd u)} }{ \int_{\zeta}^{\infty}{ \mu_n(\dd u)} - \int_{\zeta}^{\infty}{ \mu_{k_l}(\dd u)} }.
\label{eq:first_order_condition_optimality}
\end{align}
In addition we have 
\begin{align*}
&0 \leq y-\zeta=\frac{ c_n(\zeta) - c_{k_l}(\zeta) }{ \int_{\zeta}^{\infty}{ \mu_n(\dd u)} - \int_{\zeta}^{\infty}{ \mu_{k_l}(\dd u)} } \\
\Longrightarrow \quad & \int_{\zeta}^{\infty}{ \mu_n(\dd u)} -  \int_{\zeta}^{\infty}{ \mu_{k_l}(\dd u)} \geq 0.
\end{align*}
Derivatives have to be understood in the weak sense. Differentiating \eqref{eq:first_order_condition_optimality} with respect to $y$ yields
\begin{align*}
&\zeta'(y-\zeta)\left( \frac{ \mu_n(\dd \zeta) }{ \dd \zeta } - \frac{ \mu_{k_j}(\dd \zeta) }{ \dd \zeta } \right) = \int_{\zeta}^{\infty}{ \mu_n(\dd u)} -  \int_{\zeta}^{\infty}{ \mu_{k_l}(\dd u)} \geq 0 \\
\Longrightarrow \quad & \zeta' \geq 0.
\end{align*}
\end{proof}

\begin{Example}[\cite{MadanYor}]
\label{ex:Madan_Yor}
In the case when we have
\begin{align}
b_1 \leq b_2 \leq \dots \leq b_n
\label{eq:IMRV}
\end{align}
our definitions of $\xi_i$ and $K^i$, cf. \eqref{eq:definition_xi_n} and \eqref{eq:definition_Kn}, respectively, reproduce the correct quantities, i.e. 
\begin{align}
\xi_i = b_i^{-1}, \quad i=1,\dots,n, \quad \quad K_n(y) = \mu_n^{\mathrm{HL}}([y,\infty)), %\sup_{M:M_i \sim \mu_i} \E{ \indicator{\bar{M}_n \geq y }}, \quad y>0.
\end{align}
where $\mu_n^{\mathrm{HL}}$ is the Hardy-Littlewood transform of $\mu_n$.

To see this we use the steps and results in the proof of \cite[Corollary 4.1]{Touzi_maxmax}.
Clearly, the claim is true for $i=1$. Let us assume that for some $i \in \N$ we have $\xi_j=b^{-1}_j$ and $K^j_y = \frac{c_j(b^{-1}_j(y))}{y-b^{-1}_j(y)}$ for $j \leq i$.
In this case the optimization problem for $\xi_{i+1}$ in \eqref{eq:definition_xi_n} becomes
\begin{align*}
\xi_{i+1}(y) &\in \argmin_{\zeta < y} \left\{  \frac{c_{i+1}(\zeta)}{y-\zeta} - \indicator{ \zeta>b^{-1}_i } \left[ \frac{c_{i}(\zeta)}{y-\zeta} -  \frac{c_i(b^{-1}_i(y))}{y-b^{-1}_i(y)}  \right]   \right\} \\
						 &\in \argmin_{\zeta < y} \left\{ \min_{\zeta \leq b^{-1}_i} \left( \frac{c_{i+1}(\zeta)}{y-\zeta} \right) , \min_{\zeta \geq b^{-1}_i} \left( \frac{c_{i+1}(\zeta)}{y-\zeta} -  \left[ \frac{c_{i}(\zeta)}{y-\zeta} -  \frac{c_i(b^{-1}_i(y))}{y-b^{-1}_i(y)}  \right] \right)  \right\} \\
						 &\in \argmin_{\zeta < y} \left\{ A_1, A_2  \right\}  .
\end{align*}
It is clear that $A_1=\frac{c_{i+1}(b^{-1}_{i+1}(y))}{y-b^{-1}_{i+1}(y)}$. Moreover, it is shown in \cite[Corollary 4.1]{Touzi_maxmax} that $A_2 = \frac{c_{i+1}(b_i^{-1}(y))}{y-b_i^{-1}(y)} -  \left[ \frac{c_{i}(b_i^{-1}(y))}{y-b_i^{-1}(y)} -  \frac{c_i(b^{-1}_i(y))}{y-b^{-1}_i(y)}  \right] = \frac{c_{i+1}(b_i^{-1})(y)}{y-b_i^{-1}(y)}$. Consequently, $\min \left\{ A_1, A_2  \right\}  = A_1$ and $\xi_{i+1} = b^{-1}_{i+1}, K^{i+1}_y = \frac{c_{i+1}(b^{-1}_{i+1}(y))}{y-b^{-1}_{i+1}(y)}$.
\end{Example}


==> pricing.tex <==

\section{Robust Pricing of the Barrier Option}
 
\subsection{Upper Price Bound}
 
\begin{Theorem}[Robust Upper Price Bound -- Barrier Option]
\label{thm:Robust Upper Price Bound Barrier Option}
Fix $n \in \N$. 
Let $(M_t)_{t\leq n}$ be a right-continuous martingale such that $0<M_0<y $ and $M_i \sim \mu_i, i=1,\dots,n$. 

Then
\begin{align}
\E{ \indicator{\bar{M}_n \geq y} } \leq  \sum_{i=1}^{n}\left\{ \frac{c_{\jmath_i(y)}(\xi_{\jmath_i(y)})}{y-\xi_{\jmath_i(y)}} - \frac{c_{\jmath_i(y)}(\xi_{\jmath_{i+1}(y)})}{y-\xi_{\jmath_{i+1}(y)}} \indicator{i<n}  \right\}  
\label{eq:thm_pricing_barrier} 					
\end{align}
\end{Theorem}
\begin{proof}
By our notation, we have
\begin{align*}
\E{ C_i(\xi) } = \E{ \left(M_i - \xi \right)^+ } = c_i(\xi), \quad i=1,\dots, n.
\end{align*}

By Doob's inequality we have
\begin{align*}
\E{ \indicator{\bar{M}_{i-1}<y,\bar{M}_{i}\geq y} \frac{y-M_i}{y-\xi_i} } \leq 0, \quad i=1,\dots, n.
\end{align*}

Finally, because $(M_t)_{t\leq n}$ is a martingale we have
\begin{align*}
\E{ M_{i+1}-M_i }=0, \quad i=0,\dots,n-1.
\end{align*}
Hence, \eqref{eq:thm_pricing_barrier} follows from Theorem \ref{lem:Trajectorial_Inequality_Unordered_Case} by taking expectations in \eqref{eq:lem:Trajectorial_Inequality_Unordered_Case}.
\end{proof}

%\subsection{Lower Price Bound}

==> questions.tex <==

\section{Questions and Extensions}

\begin{itemize}
	\item Let $\Delta t \to 0$. What is the least lower bound for the r.h.s. of \eqref{eq:thm_Trajectorial_Inequality_Ordered_Case_1}?
	%\item Link to \cite{TrajectorialDoob}, see also \cite[Remark 2.3]{TrajectorialDoob}?
	\item Imposing $\langle \log(S) \rangle_{t_i}\leq \Xi_i$.
\end{itemize}

==> refined_pathwise_inequality.tex <==



\subsection{Refined Pathwise Inequality, $n=3$}




%\paragraph{$n=3$}

\begin{Lemma}[Refined Trajectorial Inequality, $n=3$]
\label{lem:Refined_Trajectorial_Inequality_Jump_Case}
Let $(M_t)_{t \leq n}$ be a stochastic process such that $0<M_0<y $.

Then
\begin{alignat*}{3}
\indicator{\bar{M}_3 \geq y} \leq &&& \frac{\left( M_3 - \tilde{\xi}_3(y) \right)^+}{y-\tilde{\xi}_3(y) } - \frac{ \indicator{ \bar{M}_1 \geq y } \pp{ \tilde{\xi}_3(y) - M_2}}{y-\tilde{\xi}_3(y) }   \\
 &+&& \indicator{\bar{M}_{1} \geq y, M_{2} < \tilde{\xi}_{3}(y) } \frac{M_{3} - M_{2}}{y-\tilde{\xi}_{3}}  + \indicator{ \bar{M}_3 \geq y } \frac{y-M_3}{y-\tilde{\xi}_3(y)}
\end{alignat*}
and
\begin{alignat*}{3}
\indicator{\bar{M}_3 \geq y} \leq & && \frac{\left( M_3 - \tilde{\xi}_3(y) \right)^+}{y-\tilde{\xi}_3(y) } - \frac{ \indicator{ \bar{M}_1 \geq y } \left( M_2 - \tilde{\xi}_3(y) \right)^+}{y-\tilde{\xi}_3(y) } + \frac{  \left( M_1 - \xi_1(y) \right)^+ }{y - \xi_1(y)} \\
 & + && \indicator{ \bar{M}_1 \geq y } \frac{y-M_1}{y-\xi_1(y)} + \indicator{ \bar{M}_1<y, \bar{M}_3 \geq y } \frac{y-M_3}{y-\tilde{\xi}_3(y)} \\
 & - && \indicator{ \bar{M}_1 \geq y, M_2 > \tilde{\xi}_3(y) } \frac{M_3-M_2}{y-\tilde{\xi}_3(y)}. 
\end{alignat*}

\end{Lemma}













\begin{comment}

\begin{alignat}{3}
\indicator{\bar{M}_n \geq y} \leq &  \quad && \sum_{i=1}^{n} \left( \frac{C_{\ell_i(y)}(\xi_{\ell_i}(y))}{y-\xi_{\ell_i}(y)} +\indicator{\bar{M}_{\ell_{i-1}(y)}<y,\bar{M}_{\ell_i(y)}\geq y, \ell_i(y) \neq 0} \frac{y-M_{\ell_i(y)}}{y-\xi_{\ell_i}(y)} \right) \nonumber \\
															 & - && \sum_{i=1}^{n-1}\left( \frac{C_{\ell_i}(\xi_{\ell_{i+1}}(y))}{y-\xi_{\ell_{i+1}}(y)} + \indicator{\bar{M}_{\ell_i(y)} \geq y, M_{\ell_i(y)} \geq \xi_{\ell_{i+1}}(y), \ell_i(y) \neq 0} \frac{M_{\ell_{i+1}(y)}-M_{\ell_i(y)}}{y-\xi_{\ell_{i+1}}(y)} \right)  \nonumber \\
															 & + &&  \indicator{\alpha_2 < \xi_3(y) < \xi_1(y) < \beta_2}  F_{1,2}(\xi_3(y)) +  \indicator{\alpha_2 < \xi_1(y) <  \xi_3(y)  < \beta_2 }  G_{1,2}(\xi_3(y)) \nonumber \\
															 & + && \indicator{\bar{M}_{1} \geq y, M_{1} \in (\alpha_2, \beta_2), M_{2} < \xi_{3}(y),\alpha_2 < \xi_3(y) < \xi_1(y) < \beta_2} \frac{M_{3} - M_{2}}{y-\xi_{3}}    \nonumber \\
															 & + && \indicator{\bar{M}_{1} \geq y, M_{1} \in (\alpha_2, \beta_2), M_1 < \xi_3(y), M_{2} > \xi_{3}(y),\alpha_2 < \xi_1(y) <  \xi_3(y)  < \beta_2}  \frac{M_{2} - M_{3}}{y-\xi_{3}(y)}  .
\label{eq:lem:missing_terms_n_3}
\end{alignat}





\end{Lemma}
\begin{proof} 
Let us first consider the case $\xi_3(y)<\xi_1(y) \leq \xi_2(y)$. In this case $\ell_3(y)=3$ and $\ell_2(y)=\ell_1(y)=0$.
Furthermore, it remains to check the inequality only in the case when $F_{1,2}(\xi_3(y)) \neq 0$ which happens only if $\bar{M}_{1} \geq y, M_{1} \in (\alpha_2, \beta_2), M_{2} < \xi_{3}(y)$.
The terms are in this case
\begin{align*}
\frac{C_3(\xi_3(y))}{y-\xi_3(y)} + \frac{y-M_3}{y-\xi_3(y)} - \frac{\left( \xi_3(y) - M_2 \right)^+}{y-\xi_3(y)} + \frac{M_3-M_2}{y-\xi_3(y)} \geq 1.
\end{align*}
Note also that there is equality if $M_3 \leq \xi_3(y)$.

Now let us consider the case $\xi_2(y) \geq \xi_3(y)>\xi_1(y)$. In this case $\ell_3(y)=3$, $\ell_2(y)=1,$ and $\ell_1(y)=0$.
Furthermore, it remains to check the inequality only in the case when $G_{1,2}(\xi_3(y)) \neq 0$ which happens only if $\bar{M}_{1} \geq y, M_{1} \in (\alpha_2, \beta_2), M_{1}<\xi_3(y), M_{2} > \xi_{3}(y)$.
The terms are in this case
\begin{align*}
\frac{C_1(\xi_1(y))}{y-\xi_1(y)} + \frac{y-M_1}{y-\xi_1(y)} + \frac{C_3(\xi_3(y))}{y-\xi_3(y)} - \frac{\left(M_2 - \xi_3(y) \right)^+}{y-\xi_3(y)} + \frac{M_2-M_3}{y-\xi_3(y)} \geq 1.
\end{align*}
Note also that there is equality if $M_1 \geq \xi_1(y)$ and $M_3 \geq \xi_3(y)$.

All other cases follow from Lemma \ref{lem:Trajectorial_Inequality_Ordered_Case}.
\end{proof}

\end{comment}






The price of the hedging instruments $ \indicator{ \bar{M}_1 \geq y } \left( \tilde{\xi}_3(y) - M_2\right)^+$ and $ \indicator{ \bar{M}_1 \geq y } \left( M_2 - \tilde{\xi}_3(y) \right)^+$ is model dependent. It depends on the joint distribution of $\bar{M}_1$ and $M_2$. Denote by $f^{\mathrm{iAY}}$ and $g^{\mathrm{iAY}}$ their prices in the \cite{Brown98themaximum} embedding.
Their cost is at most zero.
These terms contain information about boundary crossings.
 
 
One major disadvantage of introducing there auxiliary hedging instruments is that they won't, in general, be traded in the market. 



==> relation_optimization_problems.tex <==

\section{Global Optimization Problem vs. Sequence of Optimization Problems }

It follows from our arguments that
\begin{align}
\sum_{i=1}^{n}\left\{ \frac{c_{\jmath_i(y)}(\xi_{\jmath_i(y)})}{y-\xi_{\jmath_i(y)}} - \frac{c_{\jmath_i(y)}(\xi_{\jmath_{i+1}(y)})}{y-\xi_{\jmath_{i+1}(y)}} \indicator{i<n}  \right\}   = K^n_y = \min_{0 \leq \zeta_1 \leq \dots \leq \zeta_n < y} 
\sum_{i=1}^{n}\left\{ \frac{c_{_i}(\zeta_{i})}{y-\zeta_{i}} - \frac{c_{i}(\zeta_{i+1})}{y-\zeta_{i+1}} \indicator{i<n}  \right\} .
\end{align}

Figure \ref{fig:relation_optimization_problems_boundary_example} illustrates this.

==> relation_to_HLOST.tex <==

\subsection{Canonical Choice of $\tau'_2$ and Relation to \cite{Touzi_maxmax}}


We have talked about the strong association between $M_n$ and $\bar{M}_n$ which yields \enquote{extreme} properties for the process $M$. 
One feature of this can be seen by taking the limit to a continuum of marginals $\left( \mu_t \right)_{t \geq 0}$ (after defining an appropriate analogue of Assumption \ref{ass:unicity_minimizers}) which yields a process which has only positive jumps and in between these jumps it is either constant or decreasing.


To sum it up, our example shows that if Assumption \ref{ass:unicity_minimizers} does not hold the optimization problem \eqref{eq:definition_xi_n} might yield the wrong stopping boundary for the embedding. 
At the same time we have also seen in Example \ref{ex:MadanYor} that Assumption \ref{ass:unicity_minimizers} is too restrictive. 
It implies continuity of $\xi_2,\dots,\xi_n$ which is used in the proof of the embedding property. However, in the \enquote{increasing mean residual value} case, cf. \eqref{eq:IMRV}, the embedding can be easily shown by noting that a discontinuity of $\xi_i$ corresponds to a gap in support of $\mu_i$. From \eqref{eq:IMRV} it follows that no mass can be placed at this \enquote{jump interval} and so in principle our proof could be adapted to cover the \cite{MadanYor} case.
More generally, if one can make sure that the embedding property is satisfied at discontinuities of the stopping boundaries, Assumption \ref{ass:unicity_minimizers}(ii) could be relaxed slightly.

%\tbd In general, law of maximum $\leq$: Follows easily from pathwise inequality in \cite{Touzi_maxmax}. 

==> sufficient_condition.tex <==


\subsection{Sufficient Condition for Assumption \ref{ass:unicity_minimizers}}


Although Assumption \ref{ass:unicity_minimizers} was convenient in the construction and proof of our main result, it has the disadvantage that it is not very explicit. 

Let $(X_1,X_2)$ be a martingale with marginals $\nu_1$ and $\nu_2$.
\cite{RePEc:arx:papers:1304.2141} consider optimal lower bounds on $\E{\left| X_1 - X_2 \right|}$ of the form $\int g \dd \nu_1 + \int h \dd \nu_2$. 
For their construction they require some condition on the difference of the distribution functions of $\nu_1$ and $\nu_2$.
In our construction we have the additional state variable of the continuously sampled maximum and our construction depends on this variable. 
Hence, the fact that Assumption \ref{ass:unicity_minimizers} features quantities which relate to this variable should not surprise.

The following result provides a class of measures for which Assumption \ref{ass:unicity_minimizers} is satisfied.

\begin{Proposition}[Sufficient Condition]
\label{prop:sufficient_condition}
Let Assumption \ref{ass:unicity_minimizers}(i) holds and assume that $c_1,\dots,c_n$ are twice differentiable. % and that there exists an $x_{\star}>\sup\left\{ x: \mu_1((x,\infty)) = 1 \right\}$ such that
%\begin{align}
%b_1(x) < b_2(x) < \dots < b_n(x) \qquad \text{for all} \quad x \leq x_{\star}.
%\end{align}

Set $\mu_0 \equiv 0$ and $l_{\mu_n} := \sup\left\{ x: \mu_n((x,\infty)) = 1 \right\}$.
Suppose that for all $\alpha = \zeta_0 \leq \zeta_{1} \leq \dots \leq \zeta_{n} = \beta$, where either $\alpha>l_{\mu_n}$ or $\beta<r_{\mu_n}$, the measures 
\begin{align}
\lambda_1 := \restr{\mu_n}{[\alpha,\beta]} \qquad \text{and} \qquad 
\lambda_2 :=  \sum_{i=0}^{n-1} \restr{\mu_i}{[\zeta_{i}, \zeta_{i+1}]}
\label{eq:restriction_measures}
\end{align}
do not have the same mass or mean or are not in convex order.

Then $\mu_1,\dots,\mu_n$ satisfy Assumption \ref{ass:unicity_minimizers}(ii).
\end{Proposition}
\begin{proof}
The case $n=2$ follows from \cite[Section 3.5]{Brown98themaximum}.
For notational convenience we will only spell out the proof in the case $n=3$.
It should be clear that similar arguments apply for general $n \in \N$.

It follows immediately that 
\begin{align*}
c_i < c_{i+1} \qquad \text{for $i=1,\dots,n-1$.}
\end{align*} 

We will proceed by proving that if $\alpha < \beta$ are minimizers in \eqref{eq:suff_cond_unicity_minimzers} then 
\begin{align}
\restr{\lambda_1}{[\alpha,\beta]} \qquad \text{and} \qquad \lambda_2 =  \restr{\mu_1}{[\alpha,\xi_2]} + \restr{\mu_2}{[\xi_2,\beta]}
\end{align}
from \eqref{eq:restriction_measures} have the same mass and mean and are in convex order. 
This situation however is ruled out by our assumption.

We restrict to the following case,
\begin{align}
\imath_3(\beta;y)=2 \qquad \text{and} \qquad \imath_3(\alpha;y)=1.
\end{align}
The other cases follow similarly. 
 
Note that under our assumptions \eqref{eq:optimality_xi} holds for $\xi_3(y) = \alpha$ and $\xi_3(y) = \beta$.
 
\textit{Masses.}
The mass of $\lambda_1$ is $c'_3(\beta) - c'_3(\alpha)$.
The mass of $\lambda_2$ is
\begin{alignat*}{3}
& &&c'_2(\beta) - c'_2(\xi_2) + c'_1(\xi_2) - c'_1(\alpha) = \stackrel{\eqref{eq:optimality_xi}}{=} c'_2(\beta) + K_2(y) - K_1(y) - c'_1(\alpha) \\ &\stackrel{\eqref{eq:optimality_xi}}{=} &&  c'_3(\beta) - c'_3(\alpha)
\end{alignat*}
where for the last equality we applied \eqref{eq:optimality_xi} for $\alpha$ and $\beta$.

\textit{Means.}
The mean of $\lambda_1$ is
\begin{align*}
\int_{\alpha}^{\beta} x \mu_3(\dd x) = c_3(\alpha) - c_3(\beta) + (\beta- \alpha) c'_3(\beta) + \underbrace{\alpha \mu_3([\alpha,\beta])}_{\mathclap{=\xi_2 \mu_3([\alpha,\beta]) - (\xi_2-\alpha) (c'_3(\beta) - c'_3(\alpha))}}.
\end{align*}
The mean of $\lambda_2$ is
\begin{alignat*}{3}
&&&c_2(\xi_2) - c_2(\beta) + (\beta- \xi_2) c'_2(\beta) + \xi_2 \mu_2([\xi_2,\beta]) \\
&+&&  c_1(\alpha) - c_1(\xi_2) + (\xi_2- \alpha) \underbrace{c'_1(\xi_2)}_{\mathclap{=\mu_1([\alpha,\xi_2]) + c'_1(\alpha)}} + \alpha \mu_1([\alpha,\xi_2]).
\end{alignat*}
Observe that by optimality of $\alpha$ and $\beta$ and smoothness we have
\begin{align*}
\frac{\partial c^3}{\partial x}(\alpha,y) = \frac{c^3(\beta,y) - c^3(\alpha,y)}{\beta-\alpha} = \frac{\partial c^3}{\partial x}(\beta,y).
\end{align*}
Now we compute the difference of the means as
\begin{alignat*}{3}
&&&c^3(\alpha,y) - c^3(\beta,y) + (\xi_2-\alpha)\frac{\partial c^3}{\partial x}(\alpha,y) + (\beta-\xi_2)\frac{\partial c^3}{\partial x}(\beta,y)  \\
&-&& (y-\alpha)K_1(y) + (y-\beta)K_2(y)  \\
&-&& (\xi_2-\alpha)c'_3(\alpha) + (\xi_2-\alpha)K_1(y) - (\alpha - \xi_2)c'_3(\beta)  + (\beta-\xi_2)K_2(y) \\
&-&& c_2(\xi_2) + c_1(\xi_2) + \alpha \mu_3([\alpha,\beta]) - \xi_2 \mu_2([\xi_2,\beta]) - \xi_2 \mu_1([\alpha, \xi_2]) \\
=&&& (y-\xi_2)K_2(y) - (y-\xi_2) K_1(y) - c_2(\xi_2) + c_1(\xi_2) \\
&-&& (\xi_2-\alpha)c'_3(\alpha) - (\alpha - \xi_2)c'_3(\beta) - (\xi_2-\alpha)(c'_3(\beta) - c'_3(\alpha)) \\
&+&& \xi_2 \big(\mu_3([\alpha,\beta] - \mu_2([\xi_2,\beta]) - \mu_1([\alpha,\xi_2)) \big) \\
=&&&0
\end{alignat*}
by definition of $K_2(y)$ and the same mass of $\lambda_1$ and $\lambda_2$.

\textit{Convex Order.}
We have to show
\begin{align*}
\int (x-z)^+ \lambda_1(\dd x) \leq \int (x-z)^+ \lambda_2(\dd x) \qquad \text{for all $z \in [\alpha,\beta]$.}
\end{align*}

We compute for $z \in [\alpha,\beta]$ 
\begin{align*}
\int (x-z)^+ \lambda_1(\dd x) = c_3(z) - c_3(\beta) - (\beta-z) \underbrace{\mu_3([\beta,\infty])}_{\mathclap{=-c'_3(\beta)}}
\end{align*}
and for  $z \in [\alpha,\xi_2]$
\begin{alignat*}{3}
\int (x-z)^+ \lambda_2(\dd x) = & &&c_1(z) - c_1(\xi_2) - (\xi_2-z) \underbrace{\mu_1([\xi_2,\infty])}_{=-c'_1(\xi_2)} \\
								 &+&&c_2(\xi_2) - c_2(\beta) - (\beta - \xi_2) \underbrace{\mu_2([\beta,\infty])}_{=-c'_2(\beta)} + (\xi_2-z) \underbrace{\mu_2([\xi_2,\beta])}_{\mathclap{=c'_2(\beta) - c'_2(\xi_2)}}.
\end{alignat*}
For $z \in [\alpha,\xi_2]$, the difference of these two expression is
\begin{alignat*}{3}
&&&\overbrace{c^3(z,y) - c^3(\beta,y) + (\beta - z) ( c'_3(\beta) - c'_2(\beta) - K_2(y) ) }^{\geq 0} \\
&+&& (y-\beta) K_2(y) -(y-\xi_2)K_1(y) + (\beta - z) K_2(y) \\
&-&& c_2(\xi_2) + c_1(\xi_2) + (\xi_2-z) \underbrace{( c'_2(\xi_2) - c'_1(\xi_2))}_{\mathclap{=-K_2(y)+K_1(y)}} \geq 0
\end{alignat*}
by definition of $K_2(y)$.

The case $z \in [\xi_2,\beta]$ follows similarly.
\end{proof}



\subsubsection{Discussion of Necessity of Proposition \ref{prop:sufficient_condition}}


The conditions in Proposition \ref{prop:sufficient_condition} seem to exclude many measures for which our construction works.

For instance, one could construct two measures with the IMRV property which violate the assumptions of Proposition \ref{prop:sufficient_condition}.



==> sufficient_condition_good.tex <==

\subsection{Characterization of Valid Iterated \AY Embeddings}

\begin{Proposition}[Characterization of Valid Iterated \AY Embeddings]
The iterated \AY yields a valid embedding if and only if the following condition on the measures $\mu_1,\dots,\mu_n$ holds:

For $y \geq 0$ denote $j=\jmath_n(y)$ and $\eta = \xi_{\jmath(y)}(y)$.
If for every $y \geq$ there exists $\zeta^{\star}$ such that
\begin{align}
c_j(\zeta^{\star}) + (\zeta^{\star} - \eta ) \bar{\mu}_j(\zeta^{\star}) = c_n(\zeta^{\star}) + (\zeta^{\star} - \eta ) \bar{\mu}_n(\zeta^{\star})
\end{align}
then the iterated \AY embedding embeds $\mu_1,\dots,\mu_n$.
\end{Proposition}

==> trajectorial_inequality.tex <==

\begin{comment}

\section{Robust Hedging of the Barrier Option}

\subsection{A Trajectorial Inequality}

The following trajectorial inequality is the building block for robust superhedging of the lookback option in the $n$-marginal case.

\begin{Lemma}[Trajectorial Inequality]
\label{lem:Trajectorial_Inequality_Ordered_Case}
Fix $n \in \N$.
Let $(M_t)_{t \leq n}$ be a stochastic process such that $0<M_0<y$ and let $0 \leq \zeta_1 \leq \dots \leq \zeta_n < y $. 

Then
\begin{alignat}{3}
\indicator{\bar{M}_n \geq y} \leq &  \quad && \sum_{i=1}^{n}\left( \frac{C_i(\zeta_i)}{y-\zeta_i} +\indicator{\bar{M}_{i-1}<y,\bar{M}_{i}\geq y} \frac{y-M_i}{y-\zeta_i} \right) \nonumber \\
															 & - && \sum_{i=1}^{n-1}\left( \frac{C_i(\zeta_{i+1})}{y-\zeta_{i+1}} + \indicator{\bar{M}_{i} \geq y, M_{i} \geq \zeta_{i+1}} \frac{M_{i+1}-M_{i}}{y-\zeta_{i+1}} \right).
\label{eq:thm_Trajectorial_Inequality_Ordered_Case_1}
\end{alignat}
\end{Lemma}


\begin{proof}
We prove the claim by induction.

The case $n=1$ is proved in \cite[Lemma 2.1]{Brown98themaximum}.

Let $n \geq 2$ and assume that the claim holds for all $n' \leq n-1$. 

First consider the case $\bar{M}_{n-1} \geq y$. By induction hypothesis,
\begin{alignat}{3}
1=\indicator{\bar{M}_n \geq y} =& \quad && \indicator{\bar{M}_{n-1} \geq y} \\
												 	 \leq & \quad && \sum_{i=1}^{n-1}\left( \frac{C_i(\zeta_i)}{y-\zeta_i} +\indicator{\bar{M}_{i-1}<y,\bar{M}_{i}\geq y} \frac{y-M_i}{y-\zeta_i} \right) \nonumber \\
																& - && \sum_{i=1}^{n-2}\left( \frac{C_i(\zeta_{i+1})}{y-\zeta_{i+1}} + \indicator{\bar{M}_{i} \geq y, M_{i} \geq \zeta_{i+1}} \frac{M_{i+1}-M_{i}}{y-\zeta_{i+1}} \right).																
\end{alignat} 
It remains to verify that the terms corresponding to $i=n$,
\begin{align}
 & \frac{C_n(\zeta_n)}{y-\zeta_n} +\indicator{\bar{M}_{n-1}<y,\bar{M}_{n}\geq y} \frac{y-M_n}{y-\zeta_n} - \left( \frac{C_{n-1}(\zeta_{n})}{y-\zeta_{n}} + \indicator{\bar{M}_{n-1} \geq y, M_{n-1} \geq \zeta_{n}} \frac{M_{n}-M_{n-1}}{y-\zeta_{n}} \right) \nonumber \\
=& \frac{C_n(\zeta_n)}{y-\zeta_n} - \left(  \frac{C_{n-1}(\zeta_{n})}{y-\zeta_{n}} + \indicator{\bar{M}_{n-1} \geq y, M_{n-1} \geq \zeta_{n}} \frac{M_{n}-M_{n-1}}{y-\zeta_{n}} \right)
\end{align}
do not destroy this inequality. Distinguishing the two case $M_{n-1}\ \geq \zeta_n$ and $M_{n-1}\ < \zeta_n$ easily shows that in both cases the contribution is non-negative.

Now consider the case $\bar{M}_{n-1} < y$. 
Observe that  
\begin{align}
\zeta \mapsto \frac{M-\zeta}{y-\zeta} \quad \text{is decreasing for $M<y$.}
\label{eq:monotonicity_call_difference}
\end{align}

We will treat the sub-cases $M_{n-1}<\zeta_n$ and $M_{n-1} \geq \zeta_n$ separately. Let us start with $M_{n-1}<\zeta_n$.
We have by induction hypothesis
\begin{alignat}{3}
0 =& \quad && \indicator{\bar{M}_{n-1} \geq y} \\
												 	 \leq & \quad && \sum_{i=1}^{n-1}\left( \frac{C_i(\zeta_i)}{y-\zeta_i} +\indicator{\bar{M}_{i-1}<y,\bar{M}_{i}\geq y} \frac{y-M_i}{y-\zeta_i} \right) \nonumber \\
																& - && \sum_{i=1}^{n-2}\left( \frac{C_i(\zeta_{i+1})}{y-\zeta_{i+1}} + \indicator{\bar{M}_{i} \geq y, M_{i} \geq \zeta_{i+1}} \frac{M_{i+1}-M_{i}}{y-\zeta_{i+1}} \right) \\
															=	& \quad && \sum_{i=1}^{n-2}\left( \underbrace{ \frac{C_i(\zeta_i)}{y-\zeta_i}  - \frac{C_i(\zeta_{i+1})}{y-\zeta_{i+1}} }_{\geq 0 \text{ by \eqref{eq:monotonicity_call_difference}}} \right) + \frac{C_{n-1}(\zeta_{n-1})}{y-\zeta_{n-1}}.
\label{eq:last_case}															
\end{alignat}
The terms corresponding to $i=n$ are
\begin{align}
 & \frac{C_n(\zeta_n)}{y-\zeta_n} +\indicator{\bar{M}_{n-1}<y,\bar{M}_{n}\geq y} \frac{y-M_n}{y-\zeta_n} - \left( \frac{C_{n-1}(\zeta_{n})}{y-\zeta_{n}} + \indicator{\bar{M}_{n-1} \geq y, M_{n-1} \geq \zeta_{n}} \frac{M_{n}-M_{n-1}}{y-\zeta_{n}} \right) \nonumber \\
=& \frac{C_n(\zeta_n)}{y-\zeta_n} +\indicator{\bar{M}_{n-1}<y,\bar{M}_{n}\geq y} \frac{y-M_n}{y-\zeta_n},
\end{align}
which contribute something non-negative in the case of $\bar{M}_n < y$ and in the case of $\bar{M}_n \geq y$ the contribution is $\frac{\left( M_n - \zeta_n \right)^+}{y-\zeta_n} + \frac{y-M_n}{y-\zeta_n} \geq 1$. 

We now treat the case $M_{n-1} \geq \zeta_n$. 
The terms corresponding to $i=n$ are in this case
\begin{align}
 & \frac{C_n(\zeta_n)}{y-\zeta_n} +\indicator{\bar{M}_{n-1}<y,\bar{M}_{n}\geq y} \frac{y-M_n}{y-\zeta_n} - \left( \frac{C_{n-1}(\zeta_{n})}{y-\zeta_{n}} + \indicator{\bar{M}_{n-1} \geq y, M_{n-1} \geq \zeta_{n}} \frac{M_{n}-M_{n-1}}{y-\zeta_{n}} \right) \nonumber \\
=& \frac{C_n(\zeta_n)}{y-\zeta_n} +\indicator{\bar{M}_{n-1}<y,\bar{M}_{n}\geq y} \frac{y-M_n}{y-\zeta_n} -  \frac{C_{n-1}(\zeta_{n})}{y-\zeta_{n}},
\end{align}
which, combined with the last term in \eqref{eq:last_case}, are at least
\begin{align}
\frac{C_n(\zeta_n)}{y-\zeta_n} +\indicator{\bar{M}_{n-1}<y,\bar{M}_{n}\geq y} \frac{y-M_n}{y-\zeta_n} + \underbrace{ \frac{C_{n-1}(\zeta_{n-1})}{y-\zeta_{n-1}} -  \frac{C_{n-1}(\zeta_{n})}{y-\zeta_{n}} }_{\geq 0 \text{ by \eqref{eq:monotonicity_call_difference}}}.
\label{eq:last_contribution}
\end{align}
Finally it remains to note that if $\bar{M}_n <y$ the contribution of \eqref{eq:last_contribution} remains non-negative, and if $\bar{M}_n \geq y$ then it is at least $\frac{\left( M_n - \zeta_n \right)^+}{ y- \zeta_n} + \frac{y-M_n}{y-\zeta_n} \geq 1$.
\end{proof}


\subsection{Financial Interpretation}
\label{subsec:Financial_Interpretation}

Interpreting the r.h.s. of \eqref{eq:thm_Trajectorial_Inequality_Ordered_Case_1} as a (pathwise) superhedging strategy for a lookback option we note that the strategy suggests entering at most one forward contract and do this only if the barrier $y$ is hit.
Furthermore, after the barrier $y$ is hit we need to rebalance the portfolio by trading in the stock at discrete time points. 

The cost today for generating the payoff $C_i(\zeta)$ at time $i$ is $c_i(\zeta)$.

\end{comment}





\section{Definitions and Preparations}

\begin{comment}
The financial interpretation of subsection \ref{subsec:Financial_Interpretation} together with 
Lemma \ref{lem:Trajectorial_Inequality_Ordered_Case} suggest that a candidate for the superhedging price of the barrier option with barrier $y$, consistent with $n$ marginal constraints, is given by
\begin{align}
\min_{0 \leq \zeta_1 \leq \dots \leq \zeta_n < y} 
\sum_{i=1}^{n}\left\{ \frac{c_{_i}(\zeta_{i})}{y-\zeta_{i}} - \frac{c_{i}(\zeta_{i+1})}{y-\zeta_{i+1}} \indicator{i<n}  \right\}  .
\label{eq:global_optimization_problem}
\end{align}

Hence, the superhedging strategy of the knock-in-digital barrier option has cost given by the expression in \eqref{eq:global_optimization_problem} and is characterized by some minimizers $\xi_1,\dots,\xi_n$ of the optimization problem \eqref{eq:global_optimization_problem}.
By setting $\zeta_i=\zeta_{i+1}$ we avoid trading in $C_i$.

\end{comment}
 
Assume that $\xi_1(y),\dots,\xi_{n-1}(y)$ and $K_y^{1},\dots,K_y^{n-1}$ are already defined. 

\begin{Definition}
\label{def:indices}
For convenience set $K^0 \equiv 0$, $C_0\equiv 0$, $c_0\equiv 0$,  $\xi_{0}\equiv -\infty$, and  $\zeta_{n+1}(y)=y = \xi_{n+1}(y)$ for $y>0$.

For $y>0$ define
\begin{equation}
\begin{split}
&\imath_n(\cdot;y): (-\infty,y] \to \left\{ 0,1,\dots,n-1 \right\}, \\ 
&\imath_n(\zeta;y) := \max \left\{k \in \{ 0,1,\dots,n-1 \}: \xi_{k}(y) < \zeta \right\},
\end{split}
\end{equation} 
and
\begin{align}
\xi_n(y) := \sup \left\{ \argmin_{\zeta < y} \left\{  \frac{c_n(\zeta)}{y-\zeta} - \left[ \frac{c_{\imath_n(\zeta;y)}(\zeta)}{y-\zeta} - K^{\imath_n(\zeta;y)}_y \right]   \right\} \right\} ,
\label{eq:definition_xi_n}
\end{align}
In addition define for $l=n-1,\dots, 1$, $y>0$,
\begin{align}
\jmath_n(y) &:= \jmath(y) := \imath_n(\xi_n(y);y), \\
\jmath_l(y) &:= \max \left\{k \in \{ 0,1,\dots,\jmath_{l+1}(y)-1 \}: \xi_{k}(y) < \xi_{\jmath_{l+1}(y)}(y) \right\} ,
\label{eq:def_ordered_indices}
\end{align} 
and
\begin{align}
K^n_y:=\frac{1}{y-\xi_n(y)} \left\{ \vphantom{\frac{1}{y-\xi_n(y)}} c_n(\xi_n(y)) - \left[ c_{\jmath(y)}(\xi_n(y)) - (y-\xi_n(y)) K^{\jmath(y)}_y \right] \right\}.
\label{eq:definition_Kn}
\end{align}
\end{Definition}

\begin{Note}
All previously defined $\xi_1,\dots,\xi_{n-1}$ remain unchanged. $\xi_n$ is defined relative to $\xi_1,\dots,\xi_{n-1}$.  
\end{Note}

With
\begin{align}
c^n(x,y):=c_n(x) - \left[ c_{\imath_n(x;y)}(x) - (y-x) K^{\imath_n(x;y)}_{y} \right]
\end{align}
the minimization problem in \eqref{eq:definition_xi_n} is equivalent to minimization of
\begin{align}
\zeta \mapsto \frac{c^n(\zeta,y)}{y-\zeta}
\end{align}
over $\zeta<y$.

Note that from the definition of $\xi_n$, $\imath_n(\cdot;y)$ and $\jmath$ it follows that if $ \zeta \mapsto \frac{c_n(\zeta)}{y-\zeta} - \left[ \frac{c_{\imath_n(\zeta;y)}(\zeta)}{y-\zeta} - K^{\imath_n(\zeta;y)}_y \right]$ is differentiable at $\xi_n(y)$, then
\begin{align}
\frac{1}{y-\xi_n(y)} K^n_y + \frac{1}{y-\xi_n(y)} \left( \vphantom{\frac{1}{y-\xi_n(y)}} c'_n(\xi_n(y)) - c'_{\jmath(y)}(\xi_n(y)) - K_y^{\jmath(y)} \right) = 0.
\label{eq:optimality_xi}
\end{align}

In the other case we have 
\begin{align}
\xi'_n(y)=0.
\label{eq:constant_xi_n}
\end{align}
This situation corresponds to an atom of $\mu_n$ and/or $\mu_{\jmath(y)}$ at $\xi_n(y)$.

\tbd We have differentiability almost everywhere.

\begin{Lemma}
The optimization problem \eqref{eq:definition_xi_n} has a solution.

In addition, for all i=1,\dots,n, the mapping
\begin{align}
\R_+ \to \R, \quad y \mapsto \xi_i(y) 
\end{align}
is non-decreasing. 
\end{Lemma}
\begin{proof}
Existence of a solution to \eqref{eq:definition_xi_n} follows from the piecewise continuity of the objective function $\zeta \mapsto \frac{c_n(\zeta)}{y-\zeta} - \left[ \frac{c_{\imath_n(\zeta;y)}(\zeta)}{y-\zeta} - K^{\imath_n(\zeta;y)}_y \right] $.

We adapt the proof of \cite[Lemma 4.6]{Touzi_maxmax}. 

Let $I_0,I_1,\dots,I_l$ and $0=k_0<k_1<\dots<k_l$, $I_0=(-\infty,\xi_{k_1}], I_l=(\xi_{k_l},y]$ be such that $\dot{ \bigcup }_{j \leq l} I_j = (-\infty,y)$ and $\restr{\imath_n(\cdot;y)}{I_j} = k_j$. 
With this notation we can rewrite the optimization problem for $\xi_n$ as 
\begin{align*}
\xi_n(y) \in \argmin 					   \left\{ \vphantom{\min_{\zeta \in (-\infty,\xi_{k_1})} \frac{c_n(\zeta)}{y-\zeta} - \left[ \frac{c_{k_0}(\zeta)}{y-\zeta} - K^{k_0}_y \right] } \right. 							& \min_{\zeta \in (-\infty,\xi_{k_1})} \frac{c_n(\zeta)}{y-\zeta} ,  \\  
																				 & \min_{\zeta \in [\xi_{k_1},\xi_{k_2})} \frac{c_n(\zeta)}{y-\zeta} - \left[ \frac{c_{k_1}(\zeta)}{y-\zeta} - K^{k_1}_y \right],	\\
																				 & \quad \quad \dots	 \\
																				 & \left. \min_{\zeta \in [\xi_{k_{l}},y)} \frac{c_n(\zeta)}{y-\zeta} - \left[ \frac{c_{k_{l}}(\zeta)}{y-\zeta} - K^{k_{l}}_y \right] \right\}.
\end{align*}
Denote by $\mathcal{H}_{\min}^{j}$ the set of interior minimizers of $\zeta \mapsto \frac{c_n(\zeta)}{y-\zeta} - \left[ \frac{c_{k_j}(\zeta)}{y-\zeta} - K^{k_j}_y \right]$ on $[\xi_{k_j}, \xi_{k_{j+1}}]$.
The first order condition for optimality is 
\begin{align}
y=\frac{ \int_{\zeta}^{\infty}{u \mu_n(\dd u)} - \int_{\zeta}^{\infty}{u \mu_{k_j}(\dd u)} }{ \int_{\zeta}^{\infty}{ \mu_n(\dd u)} - \int_{\zeta}^{\infty}{ \mu_{k_j}(\dd u)} }.
\label{eq:first_order_condition_optimality}
\end{align}
In addition we have 
\begin{align*}
&0 \leq y-\zeta=\frac{ c_n(\zeta) - c_{k_j}(\zeta) }{ \int_{\zeta}^{\infty}{ \mu_n(\dd u)} - \int_{\zeta}^{\infty}{ \mu_{k_j}(\dd u)} } \\
\Longrightarrow \quad & \int_{\zeta}^{\infty}{ \mu_n(\dd u)} -  \int_{\zeta}^{\infty}{ \mu_{k_j}(\dd u)} \geq 0.
\end{align*}
Derivatives have to be understood in the weak sense. Differentiating \eqref{eq:first_order_condition_optimality} with respect to $y$ yields
\begin{align*}
&\zeta'(y-\zeta)\left( \frac{ \mu_n(\dd \zeta) }{ \dd \zeta } - \frac{ \mu_{k_j}(\dd \zeta) }{ \dd \zeta } \right) = \int_{\zeta}^{\infty}{ \mu_n(\dd u)} -  \int_{\zeta}^{\infty}{ \mu_{k_l}(\dd u)} \geq 0 \\
\Longrightarrow \quad & \zeta' \geq 0.
\end{align*}

\tbd alternatively, BHR approach: use function $c^n$ and \enquote{tangent arguments}.
\end{proof}
 

\begin{comment}

\subsection{Robust Superhedging of the Barrier Option}

\begin{Theorem}[Robust Superhedging -- Barrier Option]
\label{lem:Trajectorial_Inequality_Unordered_Case}
Fix $n\in \N$.
Let $(M_t)_{t \leq n}$ be a stochastic process such that $0<M_0<y $.
Recall the definition of $\jmath_i$, $i=1,\dots,n,$ in equation \eqref{eq:def_ordered_indices}. 

Then
\begin{alignat}{3}
\indicator{\bar{M}_n \geq y} \leq &  \quad && \sum_{i=1}^{n} \left( \frac{C_{\jmath_i(y)}(\xi_{\jmath_i(y)})}{y-\xi_{\jmath_i(y)}} +\indicator{\bar{M}_{\jmath_{i-1}(y)}<y,\bar{M}_{\jmath_i(y)}\geq y, \jmath_i(y) \neq 0} \frac{y-M_{\jmath_i(y)}}{y-\xi_{\jmath_i(y)}} \right) \nonumber \\
															 & - && \sum_{i=1}^{n-1}\left( \frac{C_{\jmath_i}(\xi_{\jmath_{i+1}(y)})}{y-\xi_{\jmath_{i+1}(y)}} + \indicator{\bar{M}_{\jmath_i(y)} \geq y, M_{\jmath_i(y)} \geq \xi_{\jmath_{i+1}(y)}, \jmath_i \neq 0} \frac{M_{\jmath_{i+1}(y)}-M_{\jmath_i}(y)}{y-\xi_{\jmath_{i+1}(y)}} \right).
\label{eq:lem:Trajectorial_Inequality_Unordered_Case}
\end{alignat}
\end{Theorem}
\begin{proof}
This is a direct consequence of the definition of $\jmath_i$, cf. \eqref{eq:def_ordered_indices}, and Lemma \ref{lem:Trajectorial_Inequality_Ordered_Case}.
\end{proof}
 

\end{comment}

%\subsection{Subhedging}


